Learning to Generate Novel Classes for Deep Metric Learning

Deep metric learning aims to learn an embedding space where the distance between data reflects their class equivalence, even when their classes are unseen during training. However, the limited number of classes available in training precludes generalization of the learned embedding space. Motivated by this, we introduce a new data augmentation approach that synthesizes novel classes and their embedding vectors. Our approach can provide rich semantic information to an embedding model and improve its generalization by augmenting training data with novel classes unavailable in the original data. We implement this idea by learning and exploiting a conditional generative model, which, given a class label and a noise, produces a random embedding vector of the class. Our proposed generator allows the loss to use richer class relations by augmenting realistic and diverse classes, resulting in better generalization to unseen samples. Experimental results on public benchmark datasets demonstrate that our method clearly enhances the performance of proxy-based losses.

==> _4_table2_backup.tex <==
\begin{table*}[!t]
    % \scriptsize
    %\tiny
    %\small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l | c c | c c c | c c | c c c | c c | c c c} %| c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{1}{l|}{} &
    \multicolumn{5}{c|}{CUB} & \multicolumn{5}{c}{Cars} & \multicolumn{5}{|c}{SOP} %& \multicolumn{3}{|c}{In-Shop}
    \\ \cline{1-16}
    
    \multicolumn{1}{l|}{Method} & NMI & F1 & R@1 & R@2 & R@4 & NMI & F1 & R@1 & R@2 & R@4 & NMI & F1 & R@1 & R@10 & R@100 \\ 
    \hline
    
    \multicolumn{1}{l|}{Triplet} & 58.1 & 24.2 & 48.3 & 61.9 & 73.0 & 57.4 & 22.6 & 60.3 & 73.4 & 83.5 & 91.4 & 43.3 & 75.5 & 88.8 & 95.4 \\ 
    \multicolumn{1}{l|}{+ EE~\cite{ko2020embedding}}& \textbf{60.5} & \textbf{27.0} & 51.7 & 63.5 & 74.5 & \textbf{63.1} & \textbf{32.0} & 71.6 & 80.7 & 87.5 & 91.5 & 43.6 & 77.2 & 89.6 & 95.5 \\ 
    \multicolumn{1}{l|}{+ PS~\cite{gu2020proxy}}& 58.1 & 24.8 & 50.9 & 62.0 & 72.8 & 57.9 & 24.0 & 62.8 & 73.8 & 82.3 & NMI & F1 & R@1 & R@10 & R@100 \\
    
    \multicolumn{1}{l|}{+ L2A-NC} & 59.4 & 26.0 & \textbf{53.6} & \textbf{65.3} & \textbf{75.6} & 61.6 & 29.2 & \textbf{73.0} & \textbf{81.9} & \textbf{88.2} & NMI & F1 & R@1 & R@10 & R@100 \\ 
    \hline
    
    \multicolumn{1}{l|}{MS~\cite{wang2019multi}} & 62.8 & 31.2 & 56.2 & 68.3 & 79.1 & 62.4 & 30.2 & 75.0 & 83.1 & 89.5 & 91.3 & 42.7 & 75.9 & 89.3 & 95.6 \\ 
    \multicolumn{1}{l|}{+ EE~\cite{ko2020embedding}}& 63.3 & 32.5 & 57.4 & 68.7 & 79.5 & 63.5 & 33.5 & 76.1 & 84.2 & 89.8 & 91.9 & 46.1 & 78.1 & 90.3 & 95.8 \\ 
    
    \multicolumn{1}{l|}{+ PS~\cite{gu2020proxy}}& 61.1 & 29.5 & 55.9 & 68.1 & 78.1 & 58.0 & 25.0 & 71.8 & 80.9 & 87.6 & NMI & F1 & 56.4 & 74.9 & 87.3 \\ 
    
    \multicolumn{1}{l|}{+ L2A-NC} & \textbf{66.1} & \textbf{35.8} & \textbf{60.6} & \textbf{72.5} & \textbf{82.2} & \textbf{68.1} & \textbf{37.9} & \textbf{81.2} & \textbf{88.4} & \textbf{93.0} & NMI & F1 & R@1 & R@10 & R@100 \\ 
    \hline
    
    \multicolumn{1}{l|}{EE~\cite{ko2020embedding}}& \textcolor{forestgreen}{(+1.4)} & \textcolor{forestgreen}{(+2.0)} & \textcolor{forestgreen}{(+2.3)} & \textcolor{forestgreen}{(+1.0)} & \textcolor{forestgreen}{(+0.9)} & \textcolor{forestgreen}{(+3.4)} & \textcolor{forestgreen}{(+6.5)} & \textcolor{forestgreen}{(+6.1)} & \textcolor{forestgreen}{(+4.2)} & \textcolor{forestgreen}{(+2.1)} & - & - & - & - & - & 
    
    \multicolumn{1}{l|}{PS~\cite{gu2020proxy}}& \textcolor{red}{(-0.8)} & \textcolor{red}{(-0.5)} & \textcolor{forestgreen}{(+1.1)} & (0.0) & \textcolor{red}{(-0.6)} & \textcolor{red}{(-1.9)} & \textcolor{red}{(-1.9)} & \textcolor{red}{(-1.9)} & \textcolor{red}{(-0.3)} & \textcolor{red}{(-1.5)} & NMI & F1 & 56.4 & 74.9 & 87.3 & 
    
    \multicolumn{1}{l|}{L2A-NC} & \textbf{\textcolor{forestgreen}{(+2.3)}} & \textbf{\textcolor{forestgreen}{(+3.2)}} & \textbf{\textcolor{forestgreen}{(+4.9)}} & \textbf{\textcolor{forestgreen}{(+3.8)}} & \textbf{\textcolor{forestgreen}{(+2.9)}} & \textbf{\textcolor{forestgreen}{(+4.9)}} & \textbf{\textcolor{forestgreen}{(+7.1)}} & \textbf{\textcolor{forestgreen}{(+9.5)}} & \textbf{\textcolor{forestgreen}{(+6.9)}} & \textbf{\textcolor{forestgreen}{(+4.1)}} & NMI & F1 & R@1 & R@10 & R@100 &
    
    \hline
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{
        \kmc{
        Comparison with the existing pair-based losses and the state-of-the-art sample generation method, EE~\cite{ko2020embedding}. Clustering and retrieval performance are measured: NMI and F1 ($\%$), and Recall@K ($\%$), respectively. The last row denotes the average boost brought by each method.
        %$\dagger$: denotes the triplet loss equipped with the mining technique.
        }
    }
    \vspace*{-2mm}
    \label{tab:quant_pair}
\end{table*}

==> _4_table3.tex <==
\begin{table*}[!t]
    %\scriptsize
    %\tiny
    %\small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ll | c c c | c c c | c c c | c c c} %| c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{2}{l|}{} &
    \multicolumn{3}{c|}{CUB} & \multicolumn{3}{c}{Cars} & \multicolumn{3}{|c}{SOP} & \multicolumn{3}{|c}{In-Shop}
    \\
    \cline{3-14}
    
    %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100
    %\multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}
    \multicolumn{1}{l}{Method} & \multicolumn{1}{c|}{Backbone} & R@1 & R@2 & R@4 & R@1 & R@2 & R@4 & R@1 & R@10 & R@100 & R@1 & R@10 & R@20 
    \\ 
    \hline
    
    \multicolumn{1}{l}{Norm-softmax} & \multicolumn{1}{c|}{BN} & 64.9 & 76.0 & 84.3 & 83.3 & 89.7 & 94.1 & 78.6 & 90.5 & 96.0 & 90.4 & 97.7 & 98.5 &
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{BN}} & \kmc{65.2} & \kmc{75.6} & \kmc{83.7} & \kmc{83.5} & \kmc{89.7} & \kmc{93.7} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{BN} & 66.0 & 76.6 & 85.0 & 84.7 & 90.7 & 94.6 & \textbf{79.6} & 90.9 & \textbf{96.2} & 91.5 & 98.1 & 98.7 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{BN} & \textbf{66.8}  & \textbf{77.0} & \textbf{85.6} & \textbf{86.0} & \textbf{91.8} & \textbf{95.2} & 79.4 & \textbf{91.0} & \textbf{96.2} & \textbf{91.9} & \textbf{98.2} & \textbf{98.8} &
    \hline
    
    \multicolumn{1}{l}{Cosface~\cite{wang2018cosface}} & \multicolumn{1}{c|}{BN} & 65.7 & 76.2 & 84.7 & 83.6 & 89.9 & 94.2 & 78.6 & 90.4 & 95.8 & 90.7 & 97.6 & 98.3 &
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{BN}} & \kmc{64.9} & \kmc{75.2} & \kmc{83.7} & \kmc{82.9} & \kmc{89.3} & \kmc{93.4} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{BN} & 66.6 & 76.8 & 84.6 & 84.6 & 90.8 & 94.3 & \textbf{79.3} & 90.7 & 95.9 & 91.4 & 97.8 & 98.5 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{BN} & \textbf{67.6}  & \textbf{77.5} & \textbf{85.3} & \textbf{85.2} & \textbf{90.8} & \textbf{94.7} & \textbf{79.3} & \textbf{91.0} & \textbf{96.2} & \textbf{91.9} & \textbf{98.2} & \textbf{98.7} &
    \hline
    
    \multicolumn{1}{l}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{c|}{BN} & 65.1 & 76.1 & 85.0 & 83.7 & 90.4 & 94.1 & 78.1 & 90.0 & 95.9 & 90.0 & 97.7 & 98.4 &
    
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{BN}} & \kmc{66.5} & \kmc{77.0} & \kmc{85.2} & \kmc{84.1} & \kmc{90.4} & \kmc{94.2} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{BN} & 66.4 & 76.8 & 85.1 & 84.5 & 90.8 & 94.4 & 79.1 & 90.6 & 95.9 & 91.4 & 98.0 & 98.7 &
    
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{BN} & \textbf{67.7}  & \textbf{77.9} & \textbf{86.1} & \textbf{85.9} & \textbf{91.9} & \textbf{95.3} & \textbf{79.3} & \textbf{91.0} & \textbf{96.3} & \textbf{91.7} & \textbf{98.3} & \textbf{98.9} &
    \hline
    
    \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}\dagger} & \multicolumn{1}{c|}{BN} & 66.3 & 76.8 & 84.7 & 84.9 & 90.5 & 94.3 & 79.0 & 90.7 & 96.1 & 91.1 & 97.8 & 98.4 &
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{BN}} & \kmc{65.0} & \kmc{75.4} & \kmc{83.9} & \kmc{84.2} & \kmc{90.4} & \kmc{94.1} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{BN} & 66.6 & 76.8 & 85.1 & 85.3 & 91.0 & 94.8 & \textbf{79.5} & 90.6 & 96.0 & \textbf{91.8} & 98.1 & \textbf{98.7} &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{BN} & \textbf{68.0} & \textbf{78.0} & \textbf{85.4} & \textbf{86.0} & \textbf{91.4} & \textbf{95.0} & 79.4 & \textbf{91.1} & \textbf{96.3} & 91.6 & \textbf{98.2} & \textbf{98.7} &  
    \hline
    
    \multicolumn{1}{l}{Proxy-Anchor~\cite{kim2020proxy}\ddag} & \multicolumn{1}{c|}{BN} & 69.1 & 78.9 & 86.1 & 86.4 & 91.9 & 95.0 & 79.2 & 90.7 & 96.2 & 91.9 & 98.1 & 98.7 &
    \iffalse
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{BN}} & \kmc{68.9} & \kmc{78.6} & \kmc{86.2} & \kmc{86.3} & \kmc{91.7} & \kmc{95.3} & \kmc{66.6} & \kmc{80.5} & \kmc{89.5} & \kmc{87.5} & \kmc{95.9} & \kmc{97.1} &
    \fi
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{BN}} & \kmc{68.9} & \kmc{78.6} & \kmc{86.2} & \kmc{86.3} & \kmc{91.7} & \kmc{95.3} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{BN} & 69.2 & \textbf{79.5} & \textbf{87.2} & 86.9 & 92.4 & 95.2 & 79.8 & 90.9 & \textbf{96.4} &  91.9 & 98.2 & \textbf{98.8} &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{BN} & \textbf{69.7} & 79.1 & 86.4 & \textbf{87.9} & \textbf{92.8} & \textbf{95.4} & \textbf{79.9} & \textbf{91.2} & 96.1 & \textbf{92.3} & \textbf{98.3} & 98.7 &
    %\Xhline{4\arrayrulewidth}
    \hline
    
    \multicolumn{1}{l}{\kmc{Triplet}} & \multicolumn{1}{c|}{\kmc{G}} & \kmc{48.3} & \kmc{61.9} & \kmc{73.0} & \kmc{60.3} & \kmc{73.4} & \kmc{83.5} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{G}} & \kmc{51.7} & \kmc{63.5} & \kmc{74.5} & \kmc{71.6} & \kmc{80.7} & \kmc{87.5} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{\kmc{+ PS~\cite{gu2020proxy}}} & \multicolumn{1}{c|}{\kmc{G}} & \kmc{50.9} & \kmc{62.0} & \kmc{72.8} & \kmc{62.8} & \kmc{73.8} & \kmc{82.3} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{\kmc{+ L2A-NC}} & \multicolumn{1}{c|}{\kmc{G}} & \textbf{\kmc{53.6}} & \textbf{\kmc{65.3}} & \textbf{\kmc{75.6}} & \textbf{\kmc{73.0}} & \textbf{\kmc{81.9}} & \textbf{\kmc{88.2}} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    %\Xhline{4\arrayrulewidth}
    \hline
    
    \multicolumn{1}{l}{\kmc{MS~\cite{wang2019multi}}} & \multicolumn{1}{c|}{\kmc{G}} & \kmc{56.2} & \kmc{68.3} & \kmc{79.1} & \kmc{75.0} & \kmc{83.1} & \kmc{89.5} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{\kmc{+ EE~\cite{ko2020embedding}}} & \multicolumn{1}{c|}{\kmc{G}} & \kmc{57.4} & \kmc{68.7} & \kmc{79.5} & \kmc{76.1} & \kmc{84.2} & \kmc{89.8} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{\kmc{+ PS~\cite{gu2020proxy}}} & \multicolumn{1}{c|}{\kmc{G}} & \kmc{55.9} & \kmc{68.1} & \kmc{78.1} & \kmc{71.8} & \kmc{80.9} & \kmc{87.6} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    \multicolumn{1}{l}{\kmc{+ L2A-NC}} & \multicolumn{1}{c|}{\kmc{G}} & \textbf{\kmc{60.6}} & \textbf{\kmc{72.5}} & \textbf{\kmc{82.2}} & \textbf{\kmc{81.2}} & \textbf{\kmc{88.4}} & \textbf{\kmc{93.0}} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} & \kmc{-} &
    %\Xhline{4\arrayrulewidth}
    \hline
    
    \multicolumn{1}{l}{Average boost} & 
    \multicolumn{1}{c|}{EE~\cite{ko2020embedding}} & \textcolor{forestgreen}{(+0.6)} & (0.0) & (0.0) &
    \textcolor{forestgreen}{(+1.6)} & \textcolor{forestgreen}{(+1.1)} & \textcolor{forestgreen}{(+0.5)} &
    - & - & - & - & - & - &
    
    \multicolumn{1}{l}{} &
    \multicolumn{1}{c|}{PS~\cite{gu2020proxy}} & \textcolor{forestgreen}{(+0.7)} & \textcolor{forestgreen}{(+0.5)} & \textcolor{forestgreen}{(+0.4)} &
    
    \textcolor{forestgreen}{(+0.8)} & \textcolor{forestgreen}{(+0.7)} & \textcolor{forestgreen}{(+0.3)} &
    
    \textbf{\textcolor{forestgreen}{(+0.8)}} & \textcolor{forestgreen}{(+0.3)} & \textcolor{forestgreen}{(+0.1)} & %\textcolor{forestgreen}{(+0.3)} &
    
    \textcolor{forestgreen}{(+0.8)} & \textcolor{forestgreen}{(+0.3)} &
    \textcolor{forestgreen}{(+0.2)} &
    
    \multicolumn{1}{l}{} & \multicolumn{1}{c|}{L2A-NC} & \textbf{\textcolor{forestgreen}{(+1.7)}} & \textbf{\textcolor{forestgreen}{(+1.1)}} & \textbf{\textcolor{forestgreen}{(+0.8)}} &
    
    \textbf{\textcolor{forestgreen}{(+1.8)}} & \textbf{\textcolor{forestgreen}{(+1.3)}} & \textbf{\textcolor{forestgreen}{(+0.8)}} &
    
    \textbf{\textcolor{forestgreen}{(+0.8)}} & \textbf{\textcolor{forestgreen}{(+0.6)}} & \textbf{\textcolor{forestgreen}{(+0.2)}} &
    
    \textbf{\textcolor{forestgreen}{(+1.0)}}  & \textbf{\textcolor{forestgreen}{(+0.5)}} & \textbf{\textcolor{forestgreen}{(+0.3)}} &
    \hline
    
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{
        Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the public benchmark datasets. Backbone networks are denoted by abbreviations: BN for BatchNorm Inception~\cite{batchnorm} and G for GoogleNet~\cite{GoogleNet}. $\dagger$: For a fair comparison, we reproduced SoftTriple with the batch size of 128 using the author's official code and replace the original SoftTriple whose batch size is 32. $\ddag$: It is reported by the authors.  
        % Backbones of embedding networks are fixed as Inception with Batch Norm.
        %"-" means the result is not available.
        }
    \vspace*{-2mm}
    \label{tab:quant_all}
\end{table*}

==> stage1_version/_0_abstract.tex <==
% !TEX root = ./bmvc21.tex

\begin{abstract}
Deep metric learning aims to learn an embedding space where the distance between data reflects their class equivalence, even when their classes are unseen during training. However, the limited number of classes available in training precludes generalization of the learned embedding space. Motivated by this, we introduce a new data augmentation approach that synthesizes novel classes and their embedding vectors.
Our approach can provide rich semantic information to an embedding model and improve its generalization by augmenting training data with novel classes unavailable in the original data. We implement this idea by learning and exploiting a conditional generative model, which, given a class label and a noise, produces a random embedding vector of the class. Our proposed generator allows the loss to use richer class relations by augmenting realistic and diverse classes, resulting in better generalization to unseen samples. Experimental results on public benchmark datasets demonstrate that our method clearly enhances the performance of proxy-based losses.
\end{abstract}

==> stage1_version/_1_introduction.tex <==
% !TEX root = ./bmvc21.tex

\section{Introduction}
\label{sec:introduction}

Deep metric learning is the task of learning an embedding space where data of the same class are placed closely so that the distance between data reflects their class equivalence. 
It has been a driving force behind recent advances in numerous computer vision and machine learning tasks including 
image retrieval~\cite{songCVPR16,kim2019deep,Sohn_nips2016}, face identification~\cite{Chopra2005,Schroff2015}, person re-identification~\cite{Chen_2017_CVPR}, zero-shot learning~\cite{Yuan_2017_ICCV} and representation learning~\cite{kim2019deep,chen2020simple}. 
The main reason for adopting deep metric learning in these tasks is its generalization capability; the learned embedding space is expected to be well generalized to unseen classes so that it can be used to predict the class equivalence of a pair of data even when their classes are unavailable in training.

Various ways to improve performance of deep metric learning have been studied so far, such as advanced loss functions~\cite{songCVPR16,Sohn_nips2016,wang2019multi,movshovitz2017no,kim2020proxy}, ensemble methods~\cite{ensemble_embedding}, regularization techniques~\cite{JACOB_2019_ICCV}, and data augmentation by sample mining~\cite{sampling_matters,Harwood_2017_ICCV} or generation~\cite{ko2020embedding,lin2018deep}.
Although the effectiveness of these methods has been demonstrated, we believe their generalization capability could be further improved in the sense that they are inherently limited only to classes available in a training set.

\iffalse
\begin{table}
\centering
\scriptsize
\begin{tabular}{cc|cccc}
\hline
\# of classes & Average \# of samples \emph{per class} & R@1 & R@2 & R@4 & R@8 \\
\hline %\cline{2-5}
24 & 82.2 & 65.3  & 76.1 & 84.2 & 90.7 \\
49 & 40.3 & 69.6 & 79.3 & 86.8 & 92.0 \\
73 & 27.0 & 72.1 & 81.0 & 88.1 & 92.9 \\
98 & 20.1 & \textbf{74.3} & \textbf{82.9} & \textbf{89.3} & \textbf{93.9} \\
\hline
\end{tabular}
\caption{Retrieval accuracy of Proxy-Anchor versus the number of available training classes on the Cars-196 dataset.}
\label{tab:tab0}
\end{table}
\fi

\begin{figure}
\begin{tabular}{cc}
\bmvaHangBox{\includegraphics[width=4.8cm]{figure/fig1_(a).pdf}}&
\bmvaHangBox{\includegraphics[width=7.5cm]{figure/fig1_(b).pdf}}
% (a) Recall@1 on the Cars-196 &(b) Metric learning without and with L2A-NC
\end{tabular}
%\vspace{-0.5\baselineskip}
\caption{Our motivation and conceptual diagram. \textbf{Left}: Accuracy in Recall@1 versus the number of training classes with Proxy-Anchor loss on the Cars-196 dataset. The number of samples used for training is fixed. \textbf{Right}: Comparison between proxy-based metric learning with and without L2A-NC. Black, empty, and colored nodes denote proxies, real embedding vectors, and synthetic embedding vectors of augmented classes, respectively. Also, different shapes indicate different classes.}
\label{fig:fig1}
%\vspace{-4mm}
\end{figure}

\iffalse
\begin{figure}[t]
   \centering
   \includegraphics[width=0.5\columnwidth]{figure/fig1_(b).pdf}
%   \vspace{-2mm}
   \caption{
   Comparison between proxy-based metric learning with and without L2A-NC. 
   Black, empty, and solid nodes denote proxies, real embedding vectors, and synthetic embedding vectors of augmented classes, respectively. 
   Also, different shapes indicate different classes.
   The colored shades represent the decision boundary of each class. 
   L2A-NC improves the generalization of the learned embedding space by increasing inter-class variation while reducing intra-class variation.
   }
   \label{fig:fig1}
\end{figure}
\fi

% How about mention other novel class generation works, VirFace (CVPR21), and ProxySynthesis
\iffalse
\km{In this paper, we argue that the number of training classes is relatively more important than that of training samples in deep metric learning. We demonstrate the importance of the number of training classes by validating generalizaiton ability while varying the number of training classes but fixing the total number of samples used in training. As shown in Figure~\ref{fig:fig1} (left), a larger number of classes lead to better performance although the number of samples per class becomes smaller\footnote{The fixed size of training data is 1,935 and \# of samples per class is uniform.}. It is natural since more diverse classes would offer richer semantic relations between training classes. According to this observation, we remark that the existing sample generation methods for deep metric learning are limited to leverage impoverished relations between given training classes.

Recently, a method~\cite{kim2020proxy} generating additional classes is proposed, which synthesizes new classes through linear interpolation between real classes.
Although this method sheds light on the class augmentation approach distinct from existing techniques, this relatively new literature on class augmentation is yet less explored and there exists room for further improvement. Specifically, since the existing method blindly interpolates two real classes, it fails to consider other classes not involved in the interpolation. Therefore, synthetic classes may significantly overlap existing classes and can express only linear relations between real classes, which end up with duplicated and limited signals.

Motivated by aforementioned issues, we introduce a novel data augmentation method that resolves these limitations. The key idea is to synthesize novel classes and their embedding vectors through a conditional generative model, which is an auxiliary module trained together with the main embedding network. We thus call it \emph{Learning to Augment Novel Classes}, dubbed \emph{L2A-NC}. Specifically, the conditional generative model, given a class label and a noise (\ie, a latent variable), produces a random embedding vector of the class. This model is trained by a metric learning loss like the main embedding network so that the novel classes and their embedding vectors become discriminative. At the same time, it is regularized to produce realistic embedding vectors by minimizing divergence between distributions of synthetic and real embedding vectors. As a result, novel classes have distributions that fit in between those of real classes in the learned embedding space as illustrated in Fig.~\ref{fig:fig1}b. The proposed method thus can synthesize realistic and discriminative novel classes thanks to the powerful expressiveness of the generative model trained with carefully designed loss functions. Consequently, these novel classes unavailable in original data help the main embedding network to learn a better generalized embedding space. In summary, the contribution of this paper is three-fold as (1) We introduce a novel data augmentation framework for deep metric learning, called L2A-NC, which \emph{synthesizes novel classes and corresponding embedding vectors} to be augmented as additional training data through a conditional generative model. (2) We design an architecture and its training strategy that enable the generator to define novel classes and produce realistic and discriminative embedding vectors. (3) It is demonstrated on public benchmarks that L2A-NC clearly enables non-trivial performance improvement of proxy-based losses.
}
\fi

In this paper, we argue that the number of training classes is relatively more important than that of training samples in deep metric learning. We demonstrate the importance of the number of training classes by validating generalizaiton ability while varying the number of training classes but fixing the total number of samples used in training. As shown in Figure~\ref{fig:fig1} (left), a larger number of classes lead to better performance although the number of samples per class becomes smaller\footnote{The fixed size of training data is 1,935 and \# of samples per class is uniform.}. It is natural since more diverse classes would offer richer semantic relations between training classes. According to this observation, we remark that the existing sample generation methods for deep metric learning are limited to leverage impoverished relations between given training classes.

Recently, a method~\cite{kim2020proxy} generating additional classes is proposed, which synthesizes new classes through linear interpolation between real classes. Inter-class relations with synthetic classes can yield better supervisory signals beyond relations between real classes. However, since this approach greatly relies on the real classes, the generated classes cannot cover a broad range of data characteristics, resulting in limitations in improving generalization.
% Although this method sheds light on the class augmentation approach distinct from existing techniques, this relatively new literature on class augmentation is yet less explored and there exists room for further improvement. Specifically, since the existing method blindly interpolates two real classes, it fails to consider other classes not involved in the interpolation. Therefore, synthetic classes may significantly overlap existing classes and can express only linear relations between real classes, which end up with duplicated and limited signals.

In this paper, we introduce a novel data augmentation method that resolves aforementioned issues. The key idea is to synthesize novel classes and their embedding vectors through a conditional generative model, which is an auxiliary module trained together with the main embedding network. We thus call it \emph{Learning to Augment Novel Classes}, dubbed \emph{L2A-NC}. Specifically, the conditional generative model, given a class label and a noise (\ie, a latent variable), produces a random embedding vector of the class. The model is trained by a metric learning loss like the main embedding network so that the novel classes and their embedding vectors become discriminative. At the same time, it is regularized to produce realistic embedding vectors by minimizing divergence between distributions of synthetic and real embedding vectors. As a result, novel classes have distributions that fit in between those of real classes in the learned embedding space as illustrated in Fig.~\ref{fig:fig1}b. The proposed method thus can synthesize realistic and discriminative novel classes thanks to the powerful expressiveness of the generative model trained with carefully designed loss functions. Consequently, these novel classes unavailable in original data help the main embedding network to learn a better generalized embedding space. 

In summary, the contribution of this paper is three-fold as (1) We introduce a novel data augmentation framework for deep metric learning, called L2A-NC, which \emph{synthesizes novel classes and corresponding embedding vectors} to be augmented as additional training data through a conditional generative model. (2) We design an architecture and its training strategy that enable the generator to define novel classes and produce realistic and discriminative embedding vectors. (3) It is demonstrated on public benchmarks that L2A-NC clearly enables non-trivial performance improvement of proxy-based losses.

%\km{L2A-NC is clearly distinct from existing data augmentation techniques for metric learning in mainly three aspects.
%First of all, previous approaches sample or generate informative embedding vectors of existing classes while L2A-NC \emph{synthesizes novel classes and their embedding vectors} to be offered as additional training data to an embedding model. Second, existing augmentation methods are mainly designed to be coupled only with pair-based metric learning losses~\cite{Chopra2005,Schroff2015,Sohn_nips2016,wang2019multi}, yet L2A-NC is dedicated to proxy-based losses~\cite{movshovitz2017no,Qian_2019_ICCV,kim2020proxy}, more recent advances in metric learning with better empirical performance. Last but not least, compared to the recently proposed class augmentation method~\cite{gu2020proxy}, our method can synthesize more diverse and genuinely \emph{novel} classes thanks to the powerful expressiveness of our learning-based generator which optimizes a metric learning loss. Advantages of L2A-NC are empirically demonstrated on public benchmarks for deep metric learning, where it clearly improves performance of existing proxy-based methods. In summary, the contribution of this paper is three-fold as (1) We introduce a novel data augmentation framework for deep metric learning, called L2A-NC, which \emph{synthesizes novel classes and corresponding embedding vectors} to be augmented as additional training data through a conditional generative model. (2) We design an architecture and its training strategy that enable the generator to define novel classes and produce realistic and discriminative embedding vectors. (3) It is demonstrated on public benchmarks that L2A-NC clearly enables non-trivial performance improvement of proxy-based methods.
%}

\iffalse
\vspace{-2mm}
\begin{itemize}[leftmargin=*]
  \setlength\itemsep{-1mm}
  \item We introduce a novel data augmentation framework for deep metric learning, called L2A-NC, which \emph{augments training classes and corresponding embedding vectors} through a conditional generative model.
  \item We design an architecture and its training strategy that enable the generator to define novel classes and produce discriminative and realistic embedding vectors for them.
  %\item To the best of our knowledge, L2A-NC is the first data augmentation technique that can be coupled with proxy-based metric learning losses. 
  \item It is demonstrated on public benchmarks that L2A-NC enables non-trivial performance improvement of proxy-based methods and achieves state of the art when coupled with them. 
  % \item We evaluate L2A-NC on widely-used benchmark datasets for metric learning and demonstrate that it enables non-trivial performance improvement of proxy-based methods, and achieves state of the art.
  %\item We show that our proposed method is transparently applicable to existing techniques, \eg, pair-based losses, proxy-based losses, and hard sample mining. Also we demonstrate that they achieve non-trivial improvements with our method compared to those without ours.
\end{itemize}
\fi


%-------------------------------------------------------------------------

==> stage1_version/_2_relatedwork.tex <==
% !TEX root = ./bmvc21.tex

\section{Related Work}
\label{sec:relatework}

% In a large body of work on deep metric learning, most studies are divided into proposing either novel loss functions or sampling strategies. Therefore, in this section, we review loss functions and then discuss techniques for hard negative mining and generation.

% \subsection{Loss Functions for Deep Metric Learning}
% \subsection{Loss Functions for Deep Metric Learning}

% \suhac{would recommend to clearly define the concepts of ``pair-based'' and ``proxy-based'' at the beginning of this section.}

\noindent\textbf{Proxy-based losses for deep metric learning.}
The loss functions for metric learning can be categorized into two types as \emph{pair-based} and \emph{proxy-based} losses. The pair-based losses are based on the pairwise relations between data in the embedding space. However, they have high training complexity since the number of tuples increases exponentially with the number of training data, forcing a careful tuple sampling technique. 
Proxy-based losses are proposed to alleviate the complexity issue by replacing samples with a small number of proxies, which are learnable parameters representing each class.
% To alleviate the complexity issue, the concept of proxy is raised, which is a representative of each class for training data and trained as a learnable parameter. Proxy-based losses can reduce training complexity quite effectively since the number of proxies is usually much smaller than that of tuples. 
Proxy-NCA~\cite{movshovitz2017no} is the first proxy-based method which pushes a sample to its positive proxy but repels against its negative proxies. Similarly, SoftTriple~\cite{Qian_2019_ICCV} assigns multiple proxies within one class to reflect intra-class variance. Proxy-Anchor~\cite{kim2020proxy} leverages data-to-data relations via forming the anchor as proxies.

%\noindent\textbf{Loss functions for deep metric learning.}
%The loss functions for metric learning can be categorized into two types as \emph{pair-based} and \emph{proxy-based} losses. The pair-based losses are based on the pairwise relations between data in the embedding space. Contrastive loss~\cite{Chopra2005} and triplet loss~\cite{Schroff2015}, seminal examples of pair-based loss, are designed to pull similar samples and push dissimilar samples with a margin given a pair or triplet of images. N-pair loss~\cite{Sohn_nips2016} and Lifted Structure loss~\cite{songCVPR16} leverage multiple negative samples in a mini-batch.
%However, these approaches have high training complexity since the number of tuples increases exponentially with the number of training data, forcing a careful tuple sampling technique. To alleviate the complexity issue, the concept of proxy is raised, which is a representative of each class for training data and trained as a learnable parameter. Proxy-based losses can reduce training complexity quite effectively since the number of proxies is usually much smaller than that of tuples. Proxy-NCA~\cite{movshovitz2017no} is the first proxy-based method which pushes a sample to its positive proxy but repels against its negative proxies. Similarly, SoftTriple~\cite{Qian_2019_ICCV} assigns multiple proxies within one class to reflect intra-class variance. Proxy-Anchor~\cite{kim2020proxy} leverages data-to-data relations via forming the anchor as proxies.

\noindent\textbf{Sample generation for deep metric learning.}
Sample generation methods are motivated to provide potentially informative samples which do not exist in the original data. \cite{Duan_2018_CVPR,Zheng_2019_CVPR,lin2018deep} exploit generative models to synthesize synthetic embedding vectors. To reduce training complexity, \cite{ko2020embedding,gu2020symmetrical} are proposed to generate synthetic embedding vectors by simple algebraic operation in the embedding space. However, these techniques are only coupled with pair-based losses and synthesizes embedding vectors of existing classes.

\noindent\textbf{Virtual class synthesis.} Recently, several approaches to utilize virtual classes are proposed in various tasks. Virtual softmax~\cite{chen2018virtual} injects additional weight as a virtual negative class for softmax function. Proxy Synthesis~\cite{gu2020proxy} exploits virtual classes synthesized by linear interpolation between real classes. Different from them, our method synthesizes novel classes by a generative model, which utilizes the expressiveness of deep neural networks. In addition, most recently, VirFace~\cite{li2021virface} is proposed to exploit unlabeled data as samples of virtual classes. Similar to our method, this approach introduces a VAE network to generate instances of virtual classes, but it requires additional unlabeled data to train generative model.
% In contrast, our method requires no additional data other than the given labeled data.

%Create novel classes that are not directly based on real data

%However, these techniques still have a risk of losing the label information of the synthetic negative samples, and are limited in usability that they can be coupled with only pair-based losses. Whereas, our proposed method alleviates the label-losing issue since ours synthesizes novel classes via optimizing metric learning objective to reduce intra-class variation. Besides, thanks to the powerful expressiveness of the deep neural network, our synthesized classes can behave more like real classes, namely represent more complicated relations between training classes than those made by using hand-crafted features.


%Different from these methods, our method is a new data augmentation approach to synthesize novel classes and their embedding vectors so that it can provide rich supervisory signals from increased training classes, which ends up better generalization on the unseen classes during training.
% sample-level with given fixed training classes
%sampled embedding vectors are always defined within given fixed training classes, our proposed method aims to learn more robust embedding space via augmenting training classes and corresponding embedding vectors which are generated from our conditional generator.

==> stage1_version/_3_method.tex <==
% !TEX root = ./bmvc21.tex

\section{Our Approach}
\label{sec:method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figure/fig2_11.pdf}
    % \vspace{-4mm}
    \caption{
    The overall framework of L2A-NC. 
    Given a novel class label and a latent variable, the conditional generative model $g$ produces an embedding vector of the class while the main model $f$ computes that of training images.
    %While the main model $f$ computes embedding vectors of training images, $g$ generates those of  synthetic classes on the same embedding space.
    %Proxy-based loss
    In our framework, a proxy-based loss takes both of real and synthetic embedding vectors (Please refer Sec.~\ref{sec:method} for details). 
    % Note that our method can be coupled with any proxy-based loss.
    %In L2A-NC, a proxy-based loss takes both of real and synthetic embedding vectors in our framework, thus supervises $g$ as well as $f$ and makes the synthetic samples discriminative. Further, $g$ is learned to produce realistic embedding vectors by minimizing the divergence loss between distributions of real and synthetic ones (Please refer Sec.~\ref{sec:c_gen} for details). Note that our method can be coupled with any other proxy-based losses.
    }
    \label{fig:fig2}
\end{figure*}

%\st{augments the data by hallucinating embedding vectors of novel classes}
%The synthetic embedding vectors could behave like those of unseen real classes
As a way to improve generalization of deep metric learning, we propose a new data augmentation method called L2A-NC, which synthesizes novel classes and their embedding vectors.
Our method learns and utilizes a conditional generative network that models novel classes and produces their embedding vectors, which are incorporated with any proxy-based losses to help them construct a more discriminative embedding space.
%The synthetic embedding vectors could behave like real classes via , and be incorporated with any proxy-based metric learning losses to help them construct a more discriminative and better generalizable embedding space.
The overall framework of L2A-NC is illustrated in Fig.~\ref{fig:fig2}.
In the rest of this section, we review the proxy-based metric learning losses, present details of the conditional generator, describe the training procedure incorporating L2A-NC, and analyze the effectiveness of novel classes with comparison to an existing class augmentation method.

\subsection{Background: Proxy-based Losses}
%Proxy-based losses are a relatively new category of metric learning loss functions. 
%They are devised for training with low complexity by introducing the concept of proxies~\cite{movshovitz2017no}. 
%Proxies are representatives of training classes and learned together with network parameters. 
%The basic idea of proxy-based losses is to learn an embedding model by utilizing relations between samples and proxies, which represent global class information.

Suppose that we aim to learn an embedding network $f$ parameterized by $\theta_{f}$ and learnable proxies $P=[ p_{1}, p_{2}, \cdots{}, p_{C} ]$.
Let $X = [ x _{1}, x_{2}, \cdots{}, x_{N} ]$ be embedding vectors (\ie, the outputs of $f$) and $ Y = [ y_{1}, y_{2}, \cdots{}, y_{N}]$ be their corresponding labels, where $ y_{i} \in{ \{ 1, 2, .., C \} } $. 
A proxy-based loss optimized with respect to $\theta_{f}$ and $P$ is denoted by $J_{met}( X, Y, P)$.

In practice, however, proxy-based losses can be further enhanced in the sense that they are inherently limited only to training classes.
%Despite their improved performance in accuracy and speed, proxy-based losses can be further enhanced in the sense that they are inherently limited only to training classes, which would hamper generalization of the learned embedding space to unseen class data. 
From this perspective, this paper proposes a new data augmentation method to synthesize novel classes and their embedding vectors. 


\subsection{Conditional Generator}
\label{sec:c_gen}
To synthesize novel classes, we learn their proxies $ \tilde{P}=[ p_{C+1}, p_{C+2}, \cdots{}, p_{C+\tilde{C} } ] $  and a conditional generator $ g $ which produces an embedding vectors of a novel class given its label $ \tilde{y} \in{ \{ C+1, C+2, .., C+\tilde{C} \} } $ and a random noise $z$ for stochastic generation:
\begin{equation}
\tilde{x} = g(\tilde{y}, z).
\end{equation}
%The generator consists of 4 fully connected layers, and is conditioned on the class label $\tilde{y}$ via conditional batch normalization layers~\cite{de2017modulating} which are placed between every pair of fully connected layers and transform intermediate features in a class-wise manner.
Along with this conditional generation process, it is necessary to regularize our generator to produce realistic embedding vectors which are not far from the distribution of real embedding vectors; this is in line with previous data augmentation methods for deep metric learning~\cite{Schroff2015,Duan_2018_CVPR,Zheng_2019_CVPR}.
Furthermore, novel classes have to be discriminative so that they become diverse and independent to each other  like real classes of the original dataset.

%\vspace{1mm}
\noindent \textbf{Loss functions.} 
To guarantee that our generator produces realistic and discriminative embedding vectors, we introduce two loss functions for its training: A divergence loss $J_{div}$ and a proxy-based loss $J_{met}$. First, the generator is encouraged to fit its generated distributions in between those of real embedding vectors by minimizing the divergence loss.

%The divergence loss is a divergence measure between two sets of embedding vectors.

\iffalse
\begin{equation}
J_{div}( X, \tilde{X}) = d( X, \tilde{X}).
\label{eq:div_loss}
\end{equation}
\fi

%As demonstrated in literature on generative models~\cite{genevay2018learning,martin2017wasserstein}, a good candidate for the divergence measure $d$ in Eq.~\eqref{eq:div_loss} is the Wasserstein distance, which allows $J_{div}$ to be statistically consistent~\cite{salimans2018improving}. The Wasserstein distance is defined by
As demonstrated in literature on generative models~\cite{genevay2018learning,martin2017wasserstein}, a good candidate for the divergence loss is the Wasserstein distance which is known to be statistically consistent~\cite{salimans2018improving}, and is defined by
\begin{equation}
\mathcal{W}(p,q)= \inf_{\gamma \in \Pi_{(p,q)}} \mathbb{E}_{x_{p},\ x_{q} \sim \gamma } [c(x_{p},x_{q}) ],
\label{eq:w_dist}
\end{equation}
where $ \Pi{}(p,q) $ is the set of all joint distributions $ \gamma{}(x_{p},x_{q}) $ and $c(\cdot,\cdot)$ denotes a cost function. This distance is usually interpreted as the minimum cost to turn the distribution $ q $ into the distribution $ p $. However, since the optimization problem in Eq.~\eqref{eq:w_dist} is generally intractable, 
%, $\mathcal{W}_{c}$
we resort to the entropy-regularized Sinkhorn distance~\cite{cuturi2013sinkhorn}. In addition, to evaluate the Wasserstein distance on given mini-batches of $X_{p}$, $X_{q}$, we choose \textit{Sinkhorn AutoDiff}~\cite{genevay2018learning} proposed as an approximate of the distance:
\begin{equation}
    \mathcal{W}_{c}( X_{p}, X_{q})=\inf_{M \in \mathcal{M} } \Tr [M \odot  C  ],
\end{equation}
where the cost function $c$ becomes the cost matrix $C$, where $C_{i,j}=c(x^{p}_{i}, x^{q}_{j})$, and the coupling distribution $ \gamma $ becomes the soft matching matrix $M$ whose all rows and columns sum to one. Although it is able to perform efficient optimization on GPUs, its gradients become no longer an unbiased gradient estimator when using mini-batches. Therefore, we finally adopt \textit{Mini-batch Energy Distance}~\cite{salimans2018improving}, which results in unbiased mini-batch gradients, as the divergence loss which is given by
\begin{equation}
\begin{aligned}
J_{div}(X, \tilde{X}) = & 2\mathbb{E}[\mathcal{W}_{c}(X_{1}, \tilde{X}_{1}) ] - \mathbb{E}[\mathcal{W}_{c}(X_{1}, X_{2})] -\mathbb{E}[\mathcal{W}_{c}(\tilde{X}_{1}, \tilde{X}_{2})],
\end{aligned}
\label{eq:j_div}
\end{equation}
where $X$ divided into $ X_{1} $ and $ X_{2} $ is a mini-batch from real data and $\tilde{X}$ divided into $\tilde{X}_{1} $ and $\tilde{X}_{2} $ is a mini-batch from generated data. For a cost function $c$, we adopt the cosine distance.

\iffalse
\begin{equation}
    \mathcal{W}_{\textrm{sinkhorn}}(p,q)= \inf_{\gamma \in \Pi_{\beta(p,q)}} \mathbb{E}_{x_{p},\ x_{q} \sim \gamma } [ c(x_{p},x_{q}) ],
\end{equation}
where $\Pi_{\beta}$ is restricted to distributions with entropy of at least some constant $\beta$. In addition, to evaluate the distance on given mini-batches of $X_{p}$, $X_{q}$, \textit{Sinkhorn AutoDiff}~\cite{genevay2018learning} is proposed as an approximate of the distance as

\begin{equation}
    \mathcal{W}_{c}( X_{p}, X_{q})=\inf_{M \in \mathcal{M} } \Tr [M \odot  C  ],
\end{equation}
where the cost function $c$ becomes the cost matrix $C$, where $C_{i,j}=c(x^{p}_{i}, x^{q}_{j})$, and the coupling distribution $ \gamma $ becomes the soft matching matrix $M$ whose all rows and columns sum to one. Despite its strength of being able to perform efficient optimization on GPUs, its gradients become no longer an unbiased gradient estimator when using mini-batches. Therefore, to design $d$ of Eq.~\eqref{eq:div_loss}, we finally resort to \textit{Mini-batch Energy Distance}~\cite{salimans2018improving} which results in unbiased mini-batch gradients and is given by
\begin{equation}
\begin{aligned}
%\begin{split}
% d(X, \tilde{X}) = & 2\mathbb{E}[\mathcal{W}_{c}(X_{1}, \tilde{X}_{1}) ] - \mathbb{E}[\mathcal{W}_{c}(X_{1}, X_{2})] \\ & -\mathbb{E}[\mathcal{W}_{c}(\tilde{X}_{1}, \tilde{X}_{2})],
% \end{aligned}
d(X, \tilde{X}) = & 2\mathbb{E}[\mathcal{W}_{c}(X_{1}, \tilde{X}_{1}) ] - \mathbb{E}[\mathcal{W}_{c}(X_{1}, X_{2})] -\mathbb{E}[\mathcal{W}_{c}(\tilde{X}_{1}, \tilde{X}_{2})],
\end{aligned}
%\end{split}
\end{equation}
where $X$ divided into $ X_{1} $ and $ X_{2} $ is a mini-batch from real data and $\tilde{X}$ divided into $\tilde{X}_{1} $ and $\tilde{X}_{2} $ is a mini-batch from generated data. For a cost function $c$, we adopt the cosine distance between two embedding vectors.
\fi
%\begin{equation}
 %   asdf%c( x, \tilde{x} )= 1 - ||x||| over ||x||. %\inf_{M \in \mathcal{M} } \Tr [\ M \odot  C  ]\ ,
%\end{equation}
%By minimizing $ J_{div} $ equipped with Eq. (7), our generator encourages the distribution of synthetic classes to be as close as possible to that of real ones.

Second, we train the generator to produce discriminative embedding vectors. 
To this end, the generator aims to minimize a proxy-based loss that takes not only novel-class data but real-class data so that novel classes become diverse and offer richer class relations to an embedding model. Formally, the objective is given by 

\begin{equation}
J_{met}( X\cup\tilde{X}, Y\cup\tilde{Y}, P\cup\tilde{P}).
\label{eq:j_met}
\end{equation}

\iffalse
\begin{algorithm}[tb]
\caption{Learning to Augment Novel Classes (L2A-NC)}
\label{alg:algorithm}
\textbf{Input}: Real embedding vectors $ X $ whose labels are denoted as $Y$, novel-class labels $\tilde{Y}$, and random noise $Z$. \\
\textbf{Parameter}: Parameters of the embedding network $\theta_{f}$, parameters of the generator $\theta_{g}$, proxies for real classes $P$ and proxies for novel classes $\tilde{P}$ \\
% Parameters of 
\textbf{Output}: Parameters of the embedding network  $\theta_{f}$.

\begin{algorithmic}[1] %[1] enables line numbers
\STATE Pretrain $ \{ \theta_{f}, P \}$ using Eq.~\eqref{eq:eqn9}.
\STATE Initialize and pretrain $\{ \theta_{g}, \tilde{P} \}$ using Eq.~\eqref{eq:eqn10}.

% \FOR{$iter$=1 to $T$}
\WHILE{not reaching the max iterations}
    %\STATE Sample a mini-batch ($D, Y$).
    %\STATE Get real samples $X=f(D)$.
    %\STATE Sample novel-class labels $\tilde{Y}$, and latent variables $z$.
    \STATE Embed real embedding vectors $ X $ from the embedding network $f$.
    \STATE Generate embedding vectors of novel classes $\tilde{X}=g(\tilde{Y}, Z)$.
    \STATE Optimize $\{ \theta_{f}, \theta_{g}, P, \tilde{P} \}$ using Eq.~\eqref{eq:eqn11}.
    \STATE Optimize $\theta_{g}$ using Eq.~\eqref{eq:div_loss}.
% \ENDFOR
\ENDWHILE
\STATE \textbf{return} $\theta_{f}$
\end{algorithmic}
\end{algorithm}
\fi

% \input{_4_table2}



\subsection{Proxy-based Metric Learning with L2A-NC}
%, consisting of the embedding network, the proposed conditional generator, proxies for both real classes and novel classes, and several losses described above.
This section illustrates the overall pipeline of our method. 
We first pretrain the embedding function $f$ alone via a specific proxy-based loss $J_{met}$:
%
% In this section, we illustrate the overall framework of our method to augment novel classes and their embedding vectors so as to achieve our final goal which is to build an embedding space well-generalized to unseen classes. For the training procedure, we first pretrain the embedding function alone via a specific proxy-based loss $J_{met}$ as:

%\iffalse
%\begin{equation}
%\min_{\theta_{g},\tilde{P}}J_{met}( \tilde{X}, \tilde{Y}, \tilde{P}) + %\lambda_{div} J_{div}( X, \tilde{X}),
%\label{eq:eqn10}
%\end{equation}
%\fi

\begin{equation}
\min_{\theta_{f},P}J_{met}( X, Y, P).
\label{eq:eqn9}
\end{equation}
Then, we pretrain the conditional generator to optimize $J_{div}(X, \tilde{X})$ and $J_{met}(\tilde{X}, \tilde{Y}, \tilde{P})$ in advance since it is difficult for the generator to synthesize realistic and discriminative embedding vectors from scratch.
Finally, in the joint training phase, the two networks $f$ and $g$ are learned by optimizing the following common objective: 
\begin{equation}
\min_{\theta_{f},\theta_{g},P,\tilde{P}}J_{met}( X\cup\tilde{X}, Y\cup\tilde{Y}, P\cup\tilde{P}) +  \lambda_{div} J_{div}( X, \tilde{X}),
\label{eq:eqn11}
\end{equation}
where $\lambda_{div} $ is a hyperparameter to balance the two losses. Note that $J_{div}$ is optimized with respect to $\tilde{X}$ only, and encourages the generator to produce realistic embedding vectors in the joint training phase also. 

\iffalse
Then, the conditional generator is also pretrained by the following optimization so as to prepare for generating realistic and discriminative embedding vectors:
% we also pretrain the generator to prepare for realistic and discriminative generation in advance as:
\begin{equation}
\min_{\theta_{g},\tilde{P}}J_{met}( \tilde{X}, \tilde{Y}, \tilde{P}) + \lambda_{div} J_{div}( X, \tilde{X}),
\label{eq:eqn10}
\end{equation}
where $\lambda_{div} $ is a hyperparameter to balance the two losses. 
\fi

%In this pretraining stage for the generator, we exclude embedding vectors of real classes when applying $J_{met}$ since embedding vectors of novel classes which are already well-separated to those of real classes could limit signals to be offered to an embedding model in the joint training phase detailed below. 

%synthetic embedding vectors that are too well-separated sufficiently trained yet could have a negative effect on those of real classes if they are trained together by $J_{met}$. 
% we find it pertinent to exclude real embedding vectors it would somewhat invalidate the final joint training phase if embedding vectors of novel classes become discriminative from those of real classes.

%Note that the loss is optimized with respect to $\tilde{X}$ only, not $X$. % and does not back-propagate its gradients to $X$.
%Note that the loss is optimized with respect to $\tilde{X}$ only and does not back-propagate its gradients to $X$.
%In this phase also, we employ the divergence loss in Eq.~\eqref{eq:div_loss} to regularize the generator and ensure that it keeps producing realistic embedding vectors. 
% for the generator to ensure its realistic generation, though the embedding space changes at each iteration of the joint training phase. 

% \begin{figure}[t]
% \centering
% \begin{subfigure}{0.48\textwidth}
%         \includegraphics[width=\textwidth]{figure/fig3_(a).pdf}
%         \caption{Data-to-proxy relation}
% \end{subfigure}       
% \begin{subfigure}{0.48\textwidth}
%         \includegraphics[width=\textwidth]{figure/fig3_(b).pdf}
%         \caption{Proxy-to-proxy relation}
% \end{subfigure}
% \caption{Novel-class data-related cosine similarity: (a) Cosine similarity between novel-class proxies and their embeddings; (b) Cosine similarity between novel-class proxies and real-class proxies. See the text for more details.}\label{fig:ps_ours} 
% \end{figure}

\begin{figure}
\includegraphics[width=0.98\textwidth]{figure/fig3.pdf}
% \begin{tabular}{cc}
% \bmvaHangBox{\includegraphics[width=5.6cm]{figure/fig3_(a).pdf}}&
% \bmvaHangBox{\includegraphics[width=5.6cm]{figure/fig3_(b).pdf}}\\
% % (a) Data-to-proxy relation & (b) Proxy-to-proxy relation
% \end{tabular}
% \vspace{0.5em}
\caption{\textbf{Left}: Cosine similarity between proxy and data points of novel classes. \textbf{Right}: Cosine similarity between novel-class proxies and real-class proxies.}
\label{fig:ps_ours}
%\vspace{-2mm}
\end{figure}

\subsection{Analysis of L2A-NC}
% As shown in Figure~\ref{fig:fig1} (a), training with larger so more diverse classes leads a model to be more robust on unseen classes in zero-shot scenario. 
In this section, we briefly review Proxy Synthesis (PS)~\cite{gu2020proxy}, an existing class augmentation method, for comparison to L2A-NC. Next, we analyze and compare the effectiveness of novel classes synthesized by PS and ours.

%\vspace{1mm}
\noindent \textbf{Review of Proxy Synthesis (PS).}
As an existing method, PS synthesizes a pair of a novel-class proxy and corresponding embedding vector by linear interpolation between pairs of real-class proxies and corresponding embedding vectors as
\begin{equation}
(\tilde{p}_{k}, \tilde{x}_{k}) = ( I_{\lambda_{ps}}(p_{i}, p_{j}), I_{\lambda_{ps}}(x_{i}, x_{j}) )
\label{eq:ps1}
\end{equation}
where $ y_{i} \neq y_{j} $, $ \tilde{x}_{k} \in \tilde{X} $, $ \tilde{p}_{k} \in \tilde{P} $,  and $ I_{\lambda_{ps}}(a, b) = \lambda_{ps}a+(1-\lambda_{ps}b) $ is a linear interpolation function with $ \lambda_{ps} \sim Beta(\alpha, \alpha) $ for $ \alpha \in (0, \infty) $, and $ \lambda_{ps} \in [0, 1] $. 
%Next, similar to ours, the embedding network $ f $ is learned by optimizing a specific proxy-based loss with a mini-batch including synthesized novel-class proxies $\tilde{P}$ and their embedding vectors $\tilde{X}$.
% \begin{equation}
% \min_{\theta_{f},P,}J_{met}( X\cup\tilde{X}, Y\cup\tilde{Y}, P\cup\tilde{P}).
% \label{eq:ps2}
% \end{equation}

\iffalse
\begin{table}
\centering
\scriptsize
\begin{tabular}{cc|cccc}
\hline
\# of classes & Average \# of samples \emph{per class} & R@1 & R@2 & R@4 & R@8 \\
\hline %\cline{2-5}
24 & 82.2 & 65.3  & 76.1 & 84.2 & 90.7 \\
49 & 40.3 & 69.6 & 79.3 & 86.8 & 92.0 \\
73 & 27.0 & 72.1 & 81.0 & 88.1 & 92.9 \\
98 & 20.1 & \textbf{74.3} & \textbf{82.9} & \textbf{89.3} & \textbf{93.9} \\
\hline
\end{tabular}
\caption{Cosine similarity Retrieval accuracy of Proxy-Anchor versus the number of available training classes on the Cars-196 dataset.}
\label{tab:ps_vs_ours}
\end{table}

\begin{table}[]
    \tiny
    \centering
    
    \begin{tabular}{cc}
    
    \begin{minipage}{.5\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc}
        \hline
        
        Dataset & +0\% & +25\% & +50\% & +100\% & +200\% \\
        \hline
        
        CUB & 69.1 & 69.3 & 69.6 & 69.5 & \textbf{69.7} \\
        SOP & 79.2 & 79.3 & 79.5 & 79.5 & \textbf{79.9} \\
        In-Shop & 91.9 & 92.0 & 92.2 & 92.2 & \textbf{92.3} \\
        \hline
        \end{tabular}
        }
    \end{minipage} &
    
    \begin{minipage}{.5\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c|c|c}
        \hline
        $\lambda_{div} $ & Norm-softmax & Arcface & Proxy-Anchor \\
        \hline %\cline{2-5}
        
        0.1 & 85.9 & 85.7 & 87.6  \\
        1.0 & \textbf{86.0} & \textbf{86.0} & \textbf{87.9}  \\
        10.0 & 85.7 & 85.5 & 87.5  \\
        \hline
        \end{tabular}
        }
    \end{minipage} &

    (a) Recall@1 versus the number of novel
classes. & (b) Comparison between L2A-EC and L2A-NC in Recall@1.

    \end{tabular}
    %}
    \caption{Novel-class data-related cosine similarity on the CUB-200-2011 and the Cars-196 dataset with Proxy-Anchor loss. (\textbf{a}) includes similarity between novel-class proxies and their embedding vectors; (\textbf{b}) includes similarity between novel-class proxies and real-class proxies ; (\textbf{c}) includes something }
    \label{tab:ps_vs_ours2}
\end{table}
\fi

%\vspace{1mm}
\noindent \textbf{Comparison to PS on the validity of novel classes.}
As previously discussed, learning with diverse classes improves performance as they allow to provide richer semantic relations. 
In this context, we verify that the proposed method can generate semantic and diverse classes like real classes, and compare it with PS\footnote{We adopt the official code from https://github.com/navervision/proxy-synthesis}.
% In this context, we evaluate how synthesized classes are semantic and diverse like real classes and compare L2A-NC and PS. 
To this end, we consider two measures: cosine similarities between sample and corresponding proxy of novel classes, and those between novel-class proxies and real-class proxies. %The former one measures how proxies and samples of novel classes behave like those of real classes. The latter measures how diverse novel classes are based on comparison to real classes.

As shown in Figure~\ref{fig:ps_ours} (left), the similarities between generated sample and corresponding proxy by L2A-NC clearly higher than those of PS. The results suggest that new classes generated by L2A-NC preserve semantic characteristics. In contrast, the similarities of PS are negative, which indicates PS offers classes that fail to preserve their labels. 
Figure~\ref{fig:ps_ours} (right) shows that the similarities between the novel-class proxy and the real-class proxy of PS are relatively higher than ours. Even, the similarities of PS higher than 0.9 on average maximum, which suggests that novel classes of PS are highly redundant to real classes and produce limited training signals.

% In terms of similarity between proxies (shown in Figure~\ref{fig:ps_ours} (right)), both methods share similar values of average mean, which means both methods synthesize novel classes in between real classes. However, on average maximum, PS shows values higher than 0.9, which means novel classes of PS are highly redundant to real classes, which limited signals for an embedding model.


%It is because of PS's inherent characteristics which can not consider other real-class data which does not exist on a mini-batch. On the contrary, L2A-NC has values around 0.25 since ours considers other classes via metric learning objective for the generator. Therefore, ours can offer more diverse classes, which ends up with richer supervisory signals for an embedding model. For qualitative results, we refer the readers to Figure~\ref{fig:fig4}.

% to see how our generator can produce embedding vectors in between those of real classes and make them discriminative between different novel classes.


%As shown in Figure~\ref{fig:ps_ours} (left), L2A-NC shows higher similarities on both average mean and average minimum. That is, our method provides novel classes that behave more like real classes than does PS. Whereas, PS shows values under -0.2 on average minimum. It means PS always offers outliers which fail to preserve their labels so may cause noisy training. In terms of proxy-to-proxy relation (shown in Figure~\ref{fig:ps_ours} (right)), both methods share similar values of average mean. Thus, we can say that novel classes from both methods are in between real classes. However, on average maximum, proxies of PS have values higher than 0.9 on both datasets. It means PS always offers novel classes which are highly redundant to real classes, which leads to limited signals for an embedding model. It is because of PS's inherent characteristics which can not consider other real-class data which does not exist on a mini-batch. On the contrary, L2A-NC has values around 0.25 since ours considers other classes via metric learning objective for the generator. Therefore, ours can offer more diverse classes, which ends up with richer supervisory signals for an embedding model. For qualitative results, we refer the readers to Figure~\ref{fig:fig4}.% to see how our generator can produce embedding vectors in between those of real classes and make them discriminative between different novel classes.

%For inter proxy-to-proxy relation (shown in Figure~\ref{fig:ps_ours}(b)), both methods share similar values of average mean. Thus, we can say that both methods generate novel classes in between real classes via linear interpolation between real-class proxies (PS) and minimizing the divergence measure (Ours). However, on average maximum, proxies of PS have values higher than 0.9 on both datasets. This means PS always offers novel classes which are very redundant to real classes, which leads to limited signals for an embedding model. It is because of PS's inherent characteristics which can not consider other real-class data which does not exist on a mini-batch. On the contrary, L2A-NC has values around 0.25 since ours considers other classes via optimizing metric learning objective for the generator. Therefore, L2A-NC can offer more diverse classes, which ends up with richer supervisory signals for an embedding model. For further results,  we refer the readers to Figure~\ref{fig:fig4} to see how our generator can produce embedding vectors in between those of real classes and make them discriminative between different novel classes.


%The key difference between L2A-NC and Proxy Synthesis is that L2A-NC synthesizes novel-class data based on optimizing metric learning objective but Proxy Synthesis synthesizes them via linear interpolation online.

%We compute cosine similarity between a proxy and corresponding embedding vectors per each novel class. Next, we plot the values of the average mean and average 

%For further evidence, we refer the readers to Figure~\ref{fig:fig4} for qualitative results on how our generator can produce embedding vectors of novel classes in betweeen those of real classes and make them discriminative.

%Algorithm~\ref{alg:algorithm} summarizes the overall training procedure.

%For the training procedure, we first pretrain the embedding function alone via a specific proxy-based loss $J_{m}$. Next, we also pretrain proxies of novel classes and the generator to produce novel-class samples which are realistic and inter-class separable with the pretrained embedding network via $\tilde{J}_{gen}$:
%where $ \theta_{G} $, $ \theta_{n} $ and $\lambda_{div} $ are parameters of the generator, proxies for novel classes,
%where $\lambda_{div} $ is a hyperparameter to balance two losses. For $J_{novel}$, we find it pertinent to exclude real samples since generated samples that are already well-separated from real ones would not be quite useful in the joint training phase. Lastly, two networks are optimized together. In this joint training phase, the proxy-based loss for the embedding network is reformulated to include samples and proxies of novel classes as: 

%Thus, the embedding network and proxies for all classes are jointly trained with $J_{joint}$, which is our final goal to provide rich signals reflecting more diversified class relations. For the generator, we keep employing $ J_{div} $ to ensure realistic generation although the embedding space changes at each iteration. In addition, $J_{joint}$ is employed together. In other words, two networks conspire together to construct a well-clustered embedding space reflecting novel classes. Therefore, the objective of the generator in the joint training phase is as follows: 
%\begin{equation}
%J_{gen} = J_{joint} + \lambda_{div} J_{div}.
%\end{equation} Algorithm 1 describes the overall training %procedure.

%Our goal is to encourage the embedding network to exploit more diverse signals from our generated novel classes. However, while the embedding network is optimized with 

%\textbf{Generator} 

%\textbf{Embedding Network}


%\subsubsection{Generator Training}
%\subsubsection{Embedding Network Training}
%\subsection{Analysis}
%\subsubsection{OT Minimization}
%\subsubsection{DML for Generator}



==> stage1_version/_4_experiments.tex <==
% !TEX root = ./bmvc21.tex
\section{Experiments}
\label{sec:experiments}

% \subsection{Experimental Settings}
\input{_4_table1}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.8\textwidth]{figure/qualitative_small.pdf}
    \vspace{-4mm}
    \caption{Qualitative results of the vanilla Proxy-Anchor~\cite{kim2020proxy} and that combined with L2A-NC on the (a) CUB, (b) Cars, and (c) SOP datasets. Images with green boundary are correct results while those with red boundary are failure cases. 
    }
    \label{fig:fig3}
    %\vspace{-3mm}
\end{figure*}

\subsection{Setup}
%\vspace{1mm}
\noindent \textbf{Datasets.} 
Combinations of L2A-NC and proxy-based losses are evaluated on benchmark datasets for deep metric learning: CUB-200-2011 (CUB)~\cite{CUB200-2011}, Cars-196 (Cars)~\cite{krause20133d}, Stanford Online Product (SOP)~\cite{songCVPR16}, and In-shop Clothes Retrieval (In-Shop)~\cite{DeepFashion}.
For splitting training and test sets, we directly follow the widely used setting in~\cite{songCVPR16}.

%\vspace{1mm}
\noindent \textbf{Network architectures.} 
We adopt BatchNorm Inception~\cite{batchnorm} with 512 output dimension. The conditional generator consists of 4 fully connected layers; a conditional batch normalization layer~\cite{de2017modulating} is inserted between every pair of layers so that the class information is injected. Also, the dimension of input noise for the generator is fixed to 16 for all experiments.
%For fair comparisons to previous methods on deep metric learning, we adopted Inception network with batch normalization~\cite{batchnorm} pre-trained on ImageNet~\cite{Imagenet} as the backbone network of the main embedding model, and appended a fully connected layer on top of it.

%The generator consists of 4 fully connected layers, and is conditioned on the class label $\tilde{y}$ via conditional batch normalization layers~\cite{de2017modulating} which are placed between every pair of fully connected layers and transform intermediate features in a class-wise manner.
%On the other hand, the conditional generator is a multi-layer perceptron that consists of 4 fully connected layers; a conditional batch normalization layer~\cite{de2017modulating} is inserted between every pair of layers so that the class information is injected to intermediate features of the network.
%Also, its input dimension (\ie, the dimension of input noise) is fixed to 16 for all experiments. 
%Note that outputs of both networks are $\ell_2$ normalized.



\vspace{1mm}
\noindent \textbf{Details of training.} 
In the pretraining stage, the main embedding models are trained by directly following the setting (\eg batch size) presented in PS~\cite{gu2020proxy}, while the conditional generator is optimized by AdamW~\cite{adamw} with the learning rate of
\expnum{1}{4} for all datasets.
% $1e-4$ for all datasets.
In the joint training stage, the learning rate of the embedding network is set to \expnum{5}{5} for all datasets.%, while the setting for the generator is the same as that for the pretraining.

\subsection{Quantitative Results}
As summarized in Table~\ref{tab:quant_all}, we observe that L2A-NC incorporated with proxy-based losses achieves non-trivial performance boosts in all datasets. Especially, on the CUB and Cars datasets, our method outperforms vanilla method and PS~\cite{kim2020proxy} by a significant margin (about $1.7\%$ and $1.0\%$ gap on average in Recall@$1$.). However, on the SOP and In-Shop datasets, we find the tendency that performance boosts of L2A-NC decreases compared to those on the CUB and Cars datasets, though L2A-NC still shows competitive or better performance boosts than PS. We conjecture this is because the SOP and In-Shop datasets have already a lot of training classes (11,318 and 3,997, respectively) which are about 113 and 40 times compared to those of CUB or Cars. Nevertheless, compared to the baseline PS, L2A-NC achieves more performance boosts except for a case of Recall@1 on the SOP where two methods are tied.

\subsection{Qualitative Results}
We further demonstrate the superiority of L2A-NC through qualitative results of image retrieval. 
Fig.~\ref{fig:fig3} presents image retrieval examples of Proxy-Anchor loss incorporating L2A-NC and those of the vanilla Proxy-Anchor. We observe that results of the vanilla Proxy-Anchor are mostly incorrect and biased towards backgrounds rather than target objects, whereas L2A-NC enables retrieval of correct images regardless of background. For example, the vanilla version failed to retrieve even a single correct image for the Cars and SOP. However, the version incorporating L2A-NC retrieved correct images although colors or viewpoints of target objects are substantially different from that of the query. We would argue that L2A-NC functions as desired to regularize the vanilla method not to be biased towards certain prevailing features in the original dataset (\eg, background, the color of an object, and viewpoint) by augmenting novel classes unavailable in the original data. %\suhac{not very clear}

\begin{table}[!t]
\begin{minipage}[t]{0.48\linewidth}
\vspace{0.37mm}
\fontsize{6}{7.8}\selectfont
% \tiny
\centering
\begin{tabularx}{1\textwidth}{ 
   >{\centering\arraybackslash}X |
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X}
\hline
\multicolumn{1}{l|}{Dataset} & +0\% & +25\% & +50\% & +100\% & +200\% \\ \hline
\multicolumn{1}{l|}{CUB} & 69.1 & 69.3 & 69.6 & 69.5 & \textbf{69.7} \\
\multicolumn{1}{l|}{SOP}& 79.2 & 79.3 & 79.5 & 79.5 & \textbf{79.9} \\
\multicolumn{1}{l|}{In-Shop} & 91.9 & 92.0 & 92.2 & 92.2 & \textbf{92.3} \\ \hline
\end{tabularx}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\linewidth}
\vspace{0.37mm}
\fontsize{6}{7.8}\selectfont
\centering
\begin{tabularx}{1\textwidth}{ 
   >{\centering\arraybackslash}X |
   >{\centering\arraybackslash}X
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X}
  \hline
\multicolumn{1}{l|}{Dataset}  & Vanilla & L2A-EC & L2A-NC (Ours)\\ \hline
\multicolumn{1}{l|}{CUB}  & 69.1  & 69.2 & \textbf{69.7} \\ 
\multicolumn{1}{l|}{Cars} & 86.4 & 86.8  & \textbf{87.9}\\ 
\multicolumn{1}{l|}{In-Shop} & 91.9 & 91.8  & \textbf{92.3}\\ \hline
\end{tabularx}
\end{minipage}
\vspace{0.5em}
\caption{Ablation studies on proposed L2A-NC. \textbf{Left}: Recall@1 versus the number of novel classes. \textbf{Right}: Comparison between L2A-EC and L2A-NC in Recall@1.}
\label{tab:tab2}
\end{table}

\iffalse
\begin{table}[]
    \tiny
    \centering
    
    \begin{tabular}{cc}
    
    \begin{minipage}{.5\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc}
        \hline
        
        Dataset & +0\% & +25\% & +50\% & +100\% & +200\% \\
        \hline
        
        CUB & 69.1 & 69.3 & 69.6 & 69.5 & \textbf{69.7} \\
        SOP & 79.2 & 79.3 & 79.5 & 79.5 & \textbf{79.9} \\
        In-Shop & 91.9 & 92.0 & 92.2 & 92.2 & \textbf{92.3} \\
        \hline
        \end{tabular}
        }
    \end{minipage} &
    
    \begin{minipage}{.5\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccc}
        \hline
        Dataset  & Vanilla & L2A-EC & L2A-NC (Ours) \\
        \hline %\cline{2-5}
        CUB  & 69.1  & 69.2 & \textbf{69.7}      \\
        CARS & 86.4 & 86.8  & \textbf{87.9}   \\
        \hline
        \end{tabular}
        }
    \end{minipage} &
    
    \iffalse
    \begin{minipage}{.3\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c|c|c}
        \hline
        $\lambda_{div} $ & Norm-softmax & CosFace~\cite{wang2018cosface} & Proxy-Anchor~\cite{kim2020proxy} \\
        \hline %\cline{2-5}
        
        0.1 & 85.9 & 85.1 & 87.6  \\
        1.0 & \textbf{86.0} & \textbf{85.2} & \textbf{87.9}  \\
        10.0 & 85.7 & 85.1 & 87.5  \\
        \hline
        \end{tabular}
        }
    \end{minipage} &
    \fi

    (a) Recall@1 versus the number of novel
classes. & (b) Comparison between L2A-EC and L2A-NC in Recall@1.

    \end{tabular}
    %}
    \caption{Ablation studies on proposed L2A-NC. (\textbf{a}) includes something; (\textbf{b}) includes something}
    \label{tab:tab2}
\end{table}
\fi

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figure/fig5.pdf}
%   \includegraphics[width=\columnwidth]{figure/fig4_5.pdf}
  \vspace{-2mm}
   \caption{
   $t$-SNE visualizations of the learned embedding space. 
   \textbf{Left}: Embedding vectors of both real and novel classes. \textbf{Right}: Embedding vectors of novel classes only.
%   (a) Comparison of real and novel embedding vectors. (b) Comparison between novel embedding vectors
   }
    \label{fig:fig4}
\end{figure*}

\subsection{In-depth Analysis on L2A-NC}

\vspace{1mm}
\noindent \textbf{Impact of the number of novel classes.}
Thanks to the architecture of our conditional generator, L2A-NC can define and synthesize an arbitrary number of novel classes. 
To investigate the impact of the number of novel classes, we evaluate the performance of L2A-NC incorporated with Proxy-Anchor loss  on the CUB, SOP and the In-Shop while varying the number of novel classes. 
As shown in Table~\ref{tab:tab2} (left), the performance increases by adding more novel classes to some degree, but there is an upper bound of the effectiveness; 
it is natural since too many novel classes may prevent the embedding model from understanding relations between classes, leading to unstable training. In experiments, we fixed the number of novel classes for all datasets: 200\% of the number of existing classes.


\vspace{1mm}
\noindent \textbf{Importance of generating novel classes.}
To verify that our performance boost is attributed to the augmentation of embedding vectors of novel classes, we compare L2A-NC with its variant that produces synthetic embedding vectors of \textit{existing classes}; we call it L2A-EC. L2A-NC and L2A-EC are incorporated with Proxy-Anchor loss, and compared on the CUB and the Cars in terms of Recall@1. 
As shown in Table~\ref{tab:tab2} (right), L2A-EC made marginal improvement compared to L2A-NC or a slight decrease compared to the vanilla method.
These results are consistent with our hypothesis that novel classes unavailable in the original dataset would provide richer signals than existing-class data.


\begin{table}[!t]
\begin{minipage}[t]{0.46\linewidth}
% \vspace{0.37mm}
\fontsize{6}{7.8}\selectfont
% \tiny
\centering
\begin{tabularx}{1\textwidth}{ 
   >{\centering\arraybackslash}X |
   >{\centering\arraybackslash}X}
\hline
\multicolumn{1}{c|}{Class pair}& Mean of minimum KL divergence \\ \hline
\multicolumn{1}{c|}{Train--Test}& 56.7\\ 
\multicolumn{1}{c|}{Novel--Test}& \textbf{27.9}\\ \hline
\end{tabularx}
\vspace{-1\baselineskip}
\caption{Quantitative analysis about how closely training and novel classes approximate unseen test classes on the CUB.}
\label{tab:tab3}
\end{minipage}
\hfill
\begin{minipage}[t]{0.52\linewidth}
% \vspace{0.37mm}
\fontsize{6}{7.8}\selectfont
\centering
\begin{tabularx}{1\textwidth}{ 
   >{\centering\arraybackslash}X |
   >{\centering\arraybackslash}X |
   >{\centering\arraybackslash}X |
   >{\centering\arraybackslash}X}
  \hline
\multicolumn{1}{l|}{Method}  & sec / iter  &  \# of parameters & R@1 boost\\ \hline
\multicolumn{1}{l|}{Vanilla}  & 0.28  & 11.85M & -\\ 
\multicolumn{1}{l|}{PS~\cite{gu2020proxy}} & 0.37 & 11.85M & 1.1\\
\multicolumn{1}{l|}{Ours} & 0.43 & 12.24M & 1.9 \\ \hline
\end{tabularx}
\vspace{-1\baselineskip}
% \caption{Performance gains and training complexity.}
\caption{Performance boost over training complexity.}
\label{tab:tab4}
\end{minipage}
\end{table}

\iffalse
\begin{table}
\tiny
%\centering
    \label{tab:tab3}
    \begin{minipage}[c]{0.48\linewidth}
    \centering
    \begin{tabular}{l|c}
    \hline
    Class pair  & Mean of minimum KL divergence \\
    \hline
    Train--Test   & 56.7     \\
    Novel--Test   & \textbf{27.9}     \\
    \hline
    \end{tabular}
    \caption{Quantitative analysis on how closely training and novel classes approximate unseen test classes.}
    \end{minipage}
    \hfill
    \label{tab:tab4}
    \begin{minipage}[c]{0.48\linewidth}
    \centering
    \begin{tabular}{l|c|c|c}
    \hline
    Method  & sec / iter  &  \# of parameters & R@1 boost \\
    \hline
    Vanilla  & 0.28  & 11.85M & (+0.0) \\
    PS~\cite{gu2020proxy} & 0.37 & 11.85M & (+1.1)  \\
    Ours & 0.43 & 12.24M & (+1.9)  \\
    \hline
    \end{tabular}
    
    \caption{Training complexity and performance boost.}
    \end{minipage}
\end{table}
\fi

\iffalse
\vspace{1mm}
\noindent \textbf{Hyperparameter ablation study.}
\km{
We also empirically investigated the effect of $\lambda_{div}$ on the Cars dataset. We searched $ \lambda_{div} \in \{ 0.1, 1.0, 10.0 \} $ and found that the best performances from all the losses are obtained when $\lambda_{div}$ is 1.0 shown in Table~\ref{tab:tab2} (c). This result implies that both losses equally matter on performance.
}
\fi

\vspace{1mm}
\noindent \textbf{\textit{t}-SNE visualization.}
% via $t$-SNE in Figure~\ref{fig:fig4}.
% Figure~\ref{fig:fig1} shows how our generated novel classes and their embedding vectors give additional signals to the embedding network. 
To illustrate how embedding vectors of novel classes offer additional signals, we visualize the learned embedding space. As shown in Figure~\ref{fig:fig4}, the generator synthesizes embedding vectors that are realistic and discriminative. In detail, Figure~\ref{fig:fig4} (left) shows that embedding vectors of novel classes are located in between those of real classes with forming their own clusters where embedding vectors of real classes do not exist. In addition, Figure~\ref{fig:fig4} (right) shows how novel classes are discriminative each other. With these results, we demonstrate how novel classes unavailable in the original dataset can offer additional signals, which lead to better generalization on unseen classes.

%Fig.~\ref{fig:fig4}a

%In detail, by minimizing the Wasserstein distance from the real distribution, novel classes are encouraged to have distributions that fit in between those of real classes (Fig.~\ref{fig:fig4}a). 
%Also, by optimizing a metric learning objective, each novel class gets discriminative so that they become diverse like real classes (Fig.~\ref{fig:fig4}b).

%Finally, novel classes and their samples fit in between real classes, which ends up enlarging inter-class variation and reducing intra-class variation of real data.

\vspace{1mm}
\noindent \textbf{Relation between novel classes and test classes.}
%Recall that metric learning aims to find an embedding space well generalizable to unseen classes.
To demonstrate that the novel classes we generate affect the robustness on unseen classes, we investigate how well the novel and unseen test classes are aligned to each other in the learned embedding space.
Specifically, we quantify the degree of alignment through KL divergence: Each novel class is first matched with its nearest test class with the minimum KL divergence, then the minimum divergence values of all novel classes are averaged. We measure this score for training classes as well for comparison. The results in Table~\ref{tab:tab3} demonstrate that novel classes better approximate test classes than training classes even though the conditional generator of L2A-NC is not aware of test data; this suggests that the proposed method has a potential to improve the generalization of the learned embedding space. 

\vspace{1mm}
\noindent \textbf{Training complexity.}
To be a promising option for practical usage, it is quite desirable for L2A-NC to offer an appealing trade-off between performance boost and training complexity. As shown in Table~\ref{tab:tab4}\footnote{All the results were produced on a NVIDIA TITAN RTX GPU.}, compared to PS~\cite{gu2020proxy}, L2A-NC achieves about 1.7 times more performance boost averaged over every benchmark when incorporated with Proxy-NCA at the cost of only 16\% and 3\% increase in training time and parameters. This result is brought by our lightweight design: the generator consists of only a few layers and holding in memory novel-class proxies is also negligible as well.
%and addresses embedding vectors whose dimension is extremely lower than that of images, and holding in memory novel-class proxies is also negligible as well.
%In other words, thanks to our light-weight design, additional computation overhead and parameters are negligible.


==> stage1_version/_4_table1.tex <==
\iffalse
\fi

\begin{table*}[!t]
    % \scriptsize
    %\tiny
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ll | c c c | c c c | c c c | c c c} %| c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{2}{l|}{} &
    \multicolumn{3}{c|}{CUB} & \multicolumn{3}{c}{Cars} & \multicolumn{3}{|c}{SOP} & \multicolumn{3}{|c}{In-Shop}
    \\ \cline{3-14}
    
    %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100
    %\multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}
    \multicolumn{1}{l}{Method} & \multicolumn{1}{c|}{Batch} & R@1 & R@2 & R@4 & R@1 & R@2 & R@4 & R@1 & R@10 & R@100 & R@1 & R@10 & R@20 
    \\ 
    
    \hline
    
    \multicolumn{1}{l}{Norm-softmax} & \multicolumn{1}{c|}{128} & 64.9 & 76.0 & 84.3 & 83.3 & 89.7 & 94.1 & 78.6 & 90.5 & 96.0 & 90.4 & 97.7 & 98.5 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.0 & 76.6 & 85.0 & 84.7 & 90.7 & 94.6 & \textbf{79.6} & 90.9 & \textbf{96.2} & 91.5 & 98.1 & 98.7 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{66.8}  & \textbf{77.0} & \textbf{85.6} & \textbf{86.0} & \textbf{91.8} & \textbf{95.2} & 79.4 & \textbf{91.0} & \textbf{96.2} & \textbf{91.9} & \textbf{98.2} & \textbf{98.8} &
    \hline
    
    \multicolumn{1}{l}{Cosface~\cite{wang2018cosface}} & \multicolumn{1}{c|}{128} & 65.7 & 76.2 & 84.7 & 83.6 & 89.9 & 94.2 & 78.6 & 90.4 & 95.8 & 90.7 & 97.6 & 98.3 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.6 & 76.8 & 84.6 & 84.6 & 90.8 & 94.3 & \textbf{79.3} & 90.7 & 95.9 & 91.4 & 97.8 & 98.5 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{67.6}  & \textbf{77.5} & \textbf{85.3} & \textbf{85.2} & \textbf{90.8} & \textbf{94.7} & \textbf{79.3} & \textbf{91.0} & \textbf{96.2} & \textbf{91.9} & \textbf{98.2} & \textbf{98.7} &
    \hline
    
    \iffalse
    \multicolumn{1}{l}{Arcface} & \multicolumn{1}{c|}{128} & 66.1 & 76.6 & 84.8 & 83.7 & 90.0 & 94.3 & 78.8 & 90.5 & 95.9 & 91.0 & 97.7 & 98.4 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.8 & 77.4 & 85.0 & 84.7 & 91.0 & 94.8 & 79.7 & 90.9 & 96.1 & 91.7 & 98.1 & 98.7 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{67.7}  & \textbf{77.7} & \textbf{85.4} & \textbf{86.0} & \textbf{91.4} & \textbf{94.5} & - & - & - & \textbf{92.3} & \textbf{98.3} & \textbf{98.8} &
    \hline
    \fi
    
    
    %\multicolumn{1}{l|}{ProxyGML~\cite{Zhu2020ProxyGML}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 77.6 & 86.4 & 85.5 & 91.8 & 95.3 & 78.0 & 90.6 & 96.2 &
    \multicolumn{1}{l}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{c|}{128} & 65.1 & 76.1 & 85.0 & 83.7 & 90.4 & 94.1 & 78.1 & 90.0 & 95.9 & 90.0 & 97.7 & 98.4 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.4 & 76.8 & 85.1 & 84.5 & 90.8 & 94.4 & 79.1 & 90.6 & 95.9 & 91.4 & 98.0 & 98.7 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{67.7}  & \textbf{77.9} & \textbf{86.1} & \textbf{85.9} & \textbf{91.9} & \textbf{95.3} & \textbf{79.3} & \textbf{91.0} & \textbf{96.3} & \textbf{91.7} & \textbf{98.3} & \textbf{98.9} &
    \hline
    
    \iffalse
    \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{c|}{32} & 65.4 & 76.4 & 84.5 & 84.5 & 90.7 & 94.5 & 78.3 & 90.4 & 96.0 & - & - & - &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{32} & 65.5 & 75.3 & 83.2  & 84.7  & 90.3 & 94.0  & - & - & - & - & - & - &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{32} & \textbf{66.7} & \textbf{77.1} & \textbf{85.1} & \textbf{85.5} & \textbf{91.2} & \textbf{94.6} & - & - & - & - & - & - &
    \hline
    \fi
    
    \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}\dagger} & \multicolumn{1}{c|}{128} & 66.3 & 76.8 & 84.7 & 84.9 & 90.5 & 94.3 & 79.0 & 90.7 & 96.1 & 91.1 & 97.8 & 98.4 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.6 & 76.8 & 85.1 & 85.3 & 91.0 & 94.8 & \textbf{79.5} & 90.6 & 96.0 & \textbf{91.8} & 98.1 & \textbf{98.7} &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{68.0} & \textbf{78.0} & \textbf{85.4} & \textbf{86.0} & \textbf{91.4} & \textbf{95.0} & 79.4 & \textbf{91.1} & \textbf{96.3} & 91.6 & \textbf{98.2} & \textbf{98.7} &  
    \hline
    
    \multicolumn{1}{l}{Proxy-Anchor~\cite{kim2020proxy}\ddag} & \multicolumn{1}{c|}{180} & 69.1 & 78.9 & 86.1 & 86.4 & 91.9 & 95.0 & 79.2 & 90.7 & 96.2 & 91.9 & 98.1 & 98.7 & 
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{180} & 69.2 & \textbf{79.5} & \textbf{87.2} & 86.9 & 92.4 & 95.2 & 79.8 & 90.9 & \textbf{96.4} &  91.9 & 98.2 & \textbf{98.8} &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{180} & \textbf{69.7} & 79.1 & 86.4 & \textbf{87.9} & \textbf{92.8} & \textbf{95.4} & \textbf{79.9} & \textbf{91.2} & 96.1 & \textbf{92.3} & \textbf{98.3} & 98.7 &
    \hline
    
    \multicolumn{1}{l}{Average boost} & \multicolumn{1}{c|}{PS~\cite{gu2020proxy}} & \textcolor{forestgreen}{(+0.7)} & \textcolor{forestgreen}{(+0.5)} & \textcolor{forestgreen}{(+0.4)} &
    
    \textcolor{forestgreen}{(+0.8)} & \textcolor{forestgreen}{(+0.7)} & \textcolor{forestgreen}{(+0.3)} &
    
    \textbf{\textcolor{forestgreen}{(+0.8)}} & \textcolor{forestgreen}{(+0.3)} & \textcolor{forestgreen}{(+0.1)} & %\textcolor{forestgreen}{(+0.3)} &
    
    \textcolor{forestgreen}{(+0.8)} & \textcolor{forestgreen}{(+0.3)} &
    \textcolor{forestgreen}{(+0.2)} &
    
    \multicolumn{1}{l}{} & \multicolumn{1}{c|}{L2A-NC} & \textbf{\textcolor{forestgreen}{(+1.7)}} & \textbf{\textcolor{forestgreen}{(+1.1)}} & \textbf{\textcolor{forestgreen}{(+0.8)}} &
    
    \textbf{\textcolor{forestgreen}{(+1.8)}} & \textbf{\textcolor{forestgreen}{(+1.3)}} & \textbf{\textcolor{forestgreen}{(+0.8)}} &
    
    \textbf{\textcolor{forestgreen}{(+0.8)}} & \textbf{\textcolor{forestgreen}{(+0.6)}} & \textbf{\textcolor{forestgreen}{(+0.2)}} &
    
    \textbf{\textcolor{forestgreen}{(+1.0)}}  & \textbf{\textcolor{forestgreen}{(+0.5)}} & \textbf{\textcolor{forestgreen}{(+0.3)}} &
    \hline
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{
        Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the public benchmark datasets. $\dagger$: For a fair comparison, we reproduced SoftTriple with the batch size of 128 using the author's official code and replace the original SoftTriple whose batch size is 32. $\ddag$: It is reported by the authors.  
        % Backbones of embedding networks are fixed as Inception with Batch Norm.
        %"-" means the result is not available.
        }
    \vspace*{-2mm}
    \label{tab:quant_all}
\end{table*}


% \begin{table*}[!t]
%     \scriptsize
%     %\tiny
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ll | c c c | c c c | c c c | c c c} %| c c c}
%     \hline
%     %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
%     %{}
%     \multicolumn{2}{l|}{} &
%     \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c}{Cars-196} & \multicolumn{3}{|c}{SOP} & \multicolumn{3}{|c}{In-Shop}
%     \\ \cline{3-14}
    
%     %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100
%     %\multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}
%     \multicolumn{1}{l}{Method} & \multicolumn{1}{c|}{Batch} & R@1 & R@2 & R@4 & R@1 & R@2 & R@4 & R@1 & R@10 & R@100 & R@1 & R@10 & R@20 
%     \\ 
    
%     \hline
    
    
%     %\multicolumn{1}{l|}{ProxyGML~\cite{Zhu2020ProxyGML}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 77.6 & 86.4 & 85.5 & 91.8 & 95.3 & 78.0 & 90.6 & 96.2 &
%     \multicolumn{1}{l}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{c|}{128} & 65.1 & 76.1 & 85.0 & 83.7 & 90.4 & 94.1 & 78.1 & 90.0 & 95.9 & 90.0 & 97.7 & 98.4 &
%     \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.4 \textcolor{forestgreen}{(+1.3)} & 76.8 \textcolor{forestgreen}{(+0.7)} & 85.1  \textcolor{forestgreen}{(+0.1)} & 84.5 \textcolor{forestgreen}{(+0.8)} & 90.8 \textcolor{forestgreen}{(+0.4)} & 94.4 \textcolor{forestgreen}{(+0.3)}  & 79.1 & 90.6 & 95.9 & 91.4 & 98.0 & 98.7 &
%     \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{67.7 \textcolor{forestgreen}{(+2.6)}}  & \textbf{77.9 \textcolor{forestgreen}{(+1.8)}} & \textbf{86.1 \textcolor{forestgreen}{(+1.1)}} & \textbf{85.8 \textcolor{forestgreen}{(+2.1)}} & \textbf{91.8 \textcolor{forestgreen}{(+1.4)}} & \textbf{95.2 \textcolor{forestgreen}{(+1.1)}} & - & - & - & - & - & - &
%     \hline
    
    
%     \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{c|}{32} & 65.4 & 76.4 & 84.5 & 84.5 & 90.7 & 94.5 & 78.3 & 90.4 & 96.0 & - & - & - &
%     \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{32} & 65.5 \textcolor{forestgreen}{(+0.1)} & 75.3 \textcolor{red}{(-1.1)} & 83.2 \textcolor{red}{(-1.3)} & 84.7 \textcolor{forestgreen}{(+0.2)} & 90.3 \textcolor{red}{(-0.4)} & 94.0 \textcolor{red}{(-0.5)} & - & - & - & - & - & - &
%     \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{32} & \textbf{66.7 \textcolor{forestgreen}{(+1.3)}} & \textbf{77.1 \textcolor{forestgreen}{(+0.7)}} & \textbf{85.1 \textcolor{forestgreen}{(+0.6)}} & \textbf{85.5 \textcolor{forestgreen}{(+1.0)}} & \textbf{91.2 \textcolor{forestgreen}{(+0.5)}} & \textbf{94.6 \textcolor{forestgreen}{(+0.1)}} & - & - & - & - & - & - &
%     \hline
    
%     \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{c|}{128} & 66.3 & 76.8 & 84.7 & 84.9 & 90.5 & 94.3 & 79.0 & 90.7 & 96.1 & 91.1 & 97.8 & 98.4 &
%     \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.6 \textcolor{forestgreen}{(+0.3)} & 76.8 (+0.0) & 85.1 \textcolor{forestgreen}{(+0.4)} & 85.3 \textcolor{forestgreen}{(+0.4)} & 91.0 \textcolor{forestgreen}{(+0.5)} & 94.8 \textcolor{forestgreen}{(+0.5)} & 79.5 & 90.6 & 96.0 & 91.8 & 98.1 & 98.7 &
%     \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{67.9 \textcolor{forestgreen}{(+1.6)}} & \textbf{78.2 \textcolor{forestgreen}{(+1.4)}} & \textbf{85.7 \textcolor{forestgreen}{(+1.0)}} & \textbf{86.0 \textcolor{forestgreen}{(+1.1)}} & \textbf{91.3 \textcolor{forestgreen}{(+0.8)}} & \textbf{94.9 \textcolor{forestgreen}{(+0.6)}} & - & - & - &  - & - & - &  
%     \hline
    
%     \multicolumn{1}{l}{Proxy-Anchor~\cite{kim2020proxy}} & \multicolumn{1}{c|}{180} & 69.1 & 78.9 & 86.1 & 86.4 & 91.9 & 95.0 & 79.2 & 90.7 & 96.2 & 91.9 & 98.1 & 98.7 & 
%     \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{180} & 69.2 \textcolor{forestgreen}{(+0.1)} & 79.5 \textcolor{forestgreen}{(+0.6)} & \textbf{87.2 \textcolor{forestgreen}{(+1.1)}} & 86.9 \textcolor{forestgreen}{(+0.5)} & 92.4 \textcolor{forestgreen}{(+0.5)} & 95.2 \textcolor{forestgreen}{(+0.2)} & 79.8 & 90.9 & \textbf{96.4} &  91.9 & 98.2 & \textbf{98.8} &
%     \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{180} & \textbf{70.0 \textcolor{forestgreen}{(+0.9)}} & \textbf{79.7 \textcolor{forestgreen}{(+0.8)}} & 86.8 \textcolor{forestgreen}{(+0.7)} & \textbf{87.7 \textcolor{forestgreen}{(+1.3)}} & \textbf{92.5 \textcolor{forestgreen}{(+0.6)}} & \textbf{95.3 \textcolor{forestgreen}{(+0.3)}} & \textbf{79.9} & \textbf{91.2} & 96.1 & \textbf{92.3} & \textbf{98.3} & 98.7 &
%     \hline
    
%     \multicolumn{1}{l}{Average boost} & \multicolumn{1}{c|}{PS~\cite{gu2020proxy}} & \textcolor{forestgreen}{(+0.4)} & (0.0) & (0.0) & \textcolor{forestgreen}{(+0.4)} & \textcolor{forestgreen}{(+0.2)} & \textcolor{forestgreen}{(+0.1)} & - & - & - & - & - & - &
%     \multicolumn{1}{l}{} & \multicolumn{1}{c|}{L2A-NC} & \textbf{\textcolor{forestgreen}{(+1.6)}} & \textbf{\textcolor{forestgreen}{(+1.1)}} & \textbf{\textcolor{forestgreen}{(+0.8)}} & \textbf{\textcolor{forestgreen}{(+1.3)}} & \textbf{\textcolor{forestgreen}{(+0.8)}} & \textbf{\textcolor{forestgreen}{(+0.5)}} & - & - & - & - & - & - &
%     \hline
    
    
%     \end{tabular}
%     }
%     \vspace{0.1mm}
%     \caption{
%         Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the CUB-200-2011, Cars-196 and SOP datasets. Superscripts denote embedding dimension. Backbones of embedding networks are fixed as Inception with Batch Norm abbreviated as BN.
%         %"-" means the result is not available.
%         }
%     %\vspace*{-4mm}
%     \label{tab:quant_all}
% \end{table*}

\iffalse
\fi

==> stage1_version/_4_table2.tex <==
\begin{table*}[!t]
    \centering
    \begin{tabular}{ll|c c c |c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{2}{l|}{\multirow{}{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196}
       & \multicolumn{3}{c}{SOP}
    \\ \cline{3-11}
    
    %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100 
    \multicolumn{2}{l|}{} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100 
    \\ \hline
    
    
    %Clustering~\cite{songCVPR17} & 48.2 & 61.4 & 71.8 & 58.1 & 70.6 & 80.3 & 67.0 & 83.7 & 93.2 &
    \multicolumn{1}{l|}{Clustering~\cite{songCVPR17}}& \multicolumn{1}{l|}{BN$^{64}$} & 48.2 & 61.4 & 71.8 & 58.1 & 70.6 & 80.3 & 67.0 & 83.7 & 93.2 &
    \multicolumn{1}{l|}{Smart Mining~\cite{Harwood_2017_ICCV}} & \multicolumn{1}{l|}{BN$^{64}$} & 49.8 & 62.3 & 74.1 & 64.7 & 76.2 & 84.2 & - & - & - & 
    \multicolumn{1}{l|}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{l|}{BN$^{64}$} & 49.2 & 61.9 & 67.9 & 73.2 & 82.4 & 86.4 & 73.7 & - & - & 
    \multicolumn{1}{l|}{Proxy-NCA + L2A-NC} & \multicolumn{1}{l|}{BN$^{64}$} & 50.8 & 62.9 & 73.0 & 73.8 & 82.4 & 88.6 & 74.3 & 87.9 & 94.7 & 
    \multicolumn{1}{l|}{Proxy-Anchor~\cite{kim2020proxy} } & \multicolumn{1}{l|}{BN$^{64}$} & 61.7 & 73.0 & 81.8 & 78.8 & 87.0 & 92.2 & 76.5 & 89.0 & 95.1 & 
    \multicolumn{1}{l|}{Proxy-Anchor + L2A-NC} & \multicolumn{1}{l|}{BN$^{64}$} & \textbf{62.6} & \textbf{73.4} & \textbf{82.1} & \textbf{80.4} & \textbf{87.7} & \textbf{92.4} & \textbf{76.7} & \textbf{89.0} & \textbf{95.1} \\
    \hline
    #\fi
    
    %Margin$^{128}$~\cite{sampling_matters} & 63.6 & 74.4 & 83.1 & 79.6 & 86.5 & 91.9 & 72.7 & 86.2 & 93.8 &
    \multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}& 57.1 & 68.8 & 78.7 & 81.4 & 88.0 & 92.7 & 74.8 & 88.3 & 94.8 &
    \multicolumn{1}{l|}{RLL-H~\cite{wang2019ranked}} & \multicolumn{1}{l|}{BN$^{512}$} & 57.4 & 69.7 & 79.2 & 74.0 & 83.6 & 90.1 & 76.1 & 89.1 & 95.4 &
    \multicolumn{1}{l|}{MS~\cite{wang2019multi}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.7 & 77.0 & 86.3 & 84.1 & 90.4 & 94.0 & 78.2 & 90.5 & 96.0 &
    %\multicolumn{1}{l|}{ProxyGML~\cite{Zhu2020ProxyGML}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 77.6 & 86.4 & 85.5 & 91.8 & 95.3 & 78.0 & 90.6 & 96.2 &
    \multicolumn{1}{l|}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.4 & 76.4 & 84.5 & 84.5 & 90.7 & 94.5 & 78.3 & 90.3 & 95.9 & 
    \multicolumn{1}{l|}{SoftTriple + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & 66.3 & 77.0 & 85.1 & 85.2 & 91.1 & 94.5 & 77.8 & 89.8 & 95.5 &
    \multicolumn{1}{l|}{Proxy-Anchor~\cite{kim2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 68.4 & 79.2 & 86.8 & 86.1 & 91.7 & 95.0 & 79.1 & 90.8 & 96.2 &
    \multicolumn{1}{l|}{Proxy-Anchor + PS~\cite{gu2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 69.2 & 79.5 & \textbf{87.2} & 86.9 & \textbf{92.4} & 95.2 & 79.8 & \textbf{90.9} & \textbf{96.4} &
    \multicolumn{1}{l|}{Proxy-Anchor + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{69.6} & \textbf{79.8} & 86.9 & \textbf{87.7} & \textbf{92.3} & \textbf{95.5} & \textbf{79.9} & \textbf{91.2} & \textbf{98.7} 
    \\ \hline
    \end{tabular}
    \vspace{0.1mm}
    \caption{
        Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the CUB-200-2011, Cars-196 and SOP datasets. Superscripts denote embedding dimension. Backbones of embedding networks are fixed as Inception with Batch Norm abbreviated as BN.
        %"-" means the result is not available.
        }
    \vspace*{-4mm}
    \label{tab:quant_all}
\end{table*}

==> stage1_version/_5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We have presented a novel data augmentation method for deep metric learning. 
Distinct from existing techniques, the proposed method synthesizes novel classes and their embedding vectors through a conditional generative model.
Thanks to the carefully designed loss functions and its architecture, the generator synthesizes novel classes which are realistic and discriminative so it can offer richer class relations to an embedding network. As a result, our method enabled proxy-based losses to improve the quality of learned embedding space and their retrieval performance. 


% How to utilize inherent real image characteristics?
% How to realize batch-conditional hard class or hard sample generation?

==> stage1_version/backup_4_experiemtns.tex <==
% !TEX root = ./bmvc21.tex
\section{Experiments}
\label{sec:experiments}

% \subsection{Experimental Settings}
\input{_4_table1}

\subsection{Setup}
Combinations of L2A-NC and proxy-based losses are evaluated on three benchmark datasets for deep metric learning: CUB-200-2011~\cite{CUB200-2011}, Cars-196~\cite{krause20133d} and, Stanford Online Product (SOP)~\cite{songCVPR16}. 
For splitting training and test sets, we directly follow the setting in~\cite{songCVPR16}.
% We followed~\cite{songCVPR16,Sohn_nips2016} for the training/test set spit. 
For CUB-200-2011, we use the first 100 classes and corresponding 5,864 images for training and the others for testing. 
For Cars-196, the first 98 classes and their 8,054 images are used for training and the rest are kept for testing. 
For SOP, we utilize 11,318 classes and their 59,551 images for training and the remaining classes and images are used for testing.

\iffalse % suha -- 20210120
%We evaluate our method on widely-used benchmark datasets for deep metric learning: CUB-200-2011~\cite{CUB200-2011}, Cars-196~\cite{krause20133d}, Stanford Online Product (SOP)~\cite{songCVPR16} and In-shop Clothes Retrieval (In-Shop)~\cite{DeepFashion}.
We evaluate our method on widely-used benchmark datasets for deep metric learning: CUB-200-2011~\cite{CUB200-2011}, Cars-196~\cite{krause20133d} and, Stanford Online Product (SOP)~\cite{songCVPR16}. We followed \cite{songCVPR16,Sohn_nips2016} for the training/test set spit. For CUB-200-2011, we split the first 100 classes (5,864 images) for training and the other classes (5,924 images) for testing. For Cars-196, we split the first 98 classes (8,054 images) for training and the rest classes (8,131 images) for testing. For SOP, we split 11,318 classes (59,551 images) for training and the remaining 11,316 classes (60,502 images) for testing~\cite{songCVPR16}. %For In-Shop, we split 3,997 classes (25,822 images) for training and the other classes (28,760 images) for testing~\cite{DeepFashion}.
\fi

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figure/qualitative_small.pdf}
    \vspace{-4mm}
    \caption{Qualitative results of the vanilla Proxy-Anchor~\cite{kim2020proxy} and that combined with L2A-NC on the CUB-200-2011 (a), Cars-196 (b), and SOP (c) datasets. Images with green boundary are correct results while those with red boundary are failure cases. 
    }
    \label{fig:fig3}
\end{figure*}

\subsection{Implementation Details}

\vspace{1mm}
\noindent \textbf{Network architectures.} 
For fair comparisons to previous methods on deep metric learning, we adopted Inception network with batch normalization~\cite{batchnorm} pre-trained on ImageNet~\cite{Imagenet} as the backbone network of the main embedding model, and appended a fully connected layer on top of it.
On the other hand, the conditional generator is a multi-layer perceptron that consists of 4 fully connected layers; a conditional batch normalization layer is inserted between every pair of fully connected layers so that the class information is injected to intermediate features of the network.
Also, its input dimension (\ie, the dimension of input noise) is fixed to 16 for all experiments. 
Note that outputs of both networks are $\ell_2$ normalized.

% For fair comparisons to previous methods on deep metric learning, we used Inception network with batch normalization~\cite{batchnorm} pre-trained for ImageNet classification~\cite{Imagenet} as our embedding network and added a fully connected layer whose size is in accordance with the dimensionality of embedding vectors, and \textit{L2}-normalize its output. 
%We followed the same hyper-parameters speci
% For the generator, we employ a 4-layer fully connected network. The dimensionality of latent variable is 16 across all experiments.

%The parameters $ \lambda{}_{ot} $ and $ \lambda{}_{genDML} $ are selected from the set $ \{ 1.0, 10.0  \} $.

\vspace{1mm}
\noindent \textbf{Details of training.} 
In the pretraining stage, the main embedding models are trained by directly following their original settings in the papers, while the conditional generator is optimized by AdamW~\cite{adamw} with the learning rate of
\expnum{1}{4} for all datasets.
% $1e-4$ for all datasets.
In the joint training stage, the learning rate of the embedding network is set to \expnum{5}{5} for all datasets, while the setting for the generator is the same as that for the pretraining.
% The hyper-parameter $\lambda_{div}$ is selected from the set $ \{ 0.1, 1.0, 10.0 \}$.
% For the virtue of fair comparisons, we basically follow each experimental setting for each loss function such as image preprocessing, batch size. In the joint training phase, however, we re-initialize the learning rate for the embedding network to be $ 5e^{-5} $ for all datasets. For the generator, we employ AdamW optimizer~\cite{adamw}. The generator is optimized with the learning rate of $ 10^{-4} $ for all datasets, which is also re-initialized to be $ 10^{-4} $ in the joint training phase in the same manner. The parameter $ \lambda{}_{div} $ is selected from the set $ \{ 0.1, 1.0, 10.0 \}$. 

%we employ AdamW optimizer~\cite{adamw} which adopts weight decay instead of $ L_{2} $ regularization. 

\subsection{Quantitative Results}
In this section, we compare retrieval performance of three representative proxy-based losses, Proxy-NCA~\cite{movshovitz2017no}, SoftTriple~\cite{Qian_2019_ICCV}, and Proxy-Anchor~\cite{kim2020proxy}, with and without L2A-NC. 
% In this section, we compare the image retrieval performance of existing proxy-based losses before and after our method is applied. L2A-NC is applied to three representative proxy-based losses, Proxy-NCA~\cite{movshovitz2017no}, SoftTriple~\cite{Qian_2019_ICCV}, and Proxy-Anchor~\cite{kim2020proxy}.
%
% popular
% representative
%As the results on the public datasets, CUB-200-2011, Cars-196, and SOP are summarized in Table 1,
%
% with varying embedding dimension in $ \{ 64, 512 \} $ 
As summarized in Table~\ref{tab:quant_all}, L2A-NC enables non-trivial performance improvement of these losses in general. 
Especially, on the CUB-200-2011 and Cars-196 datasets, it shows above $1.0\%$ performance boost on average in Recall@$1$. 
Moreover, the combination of Proxy-Anchor and L2A-NC achieves state of the art in Recall@$1$ for both 64 and 512 embedding dimensions on all three datasets.

% As the results on the public datasets are summarized in Table 1, L2A-NC generally achieves non-trivial performance improvement in Recall@K with a few exceptions. Especially, on the challenging datasets such as CUB-200-2011 and Cars-196, it shows above $1.0\%$ performance boost on average in Recall@1. Moreover, when applied to Proxy-Anchor~\cite{kim2020proxy}, our method even achieves state of the art Recall@1 for both 64/128 embedding dimension on all datasets.


%In all the three datasets, our method achieves non-trivial performance improvement in Recall@K except a few .

%Especially, on the challenging datasets such as CUB-200-2011 and Cars-196, it shows above $1.0\%$ performance boost on average in Recall@1. Moreover, when applied to Proxy-Anchor~\cite{kim2020proxy}, our method even achieves state of the art Recall@1 for both 64/128 embedding dimension on three datasets.

%On average, it achieved more than 1% performance improvement.

%even state of the art Recall@1 with Proxy-Anchor~\cite{kim2020proxy} in both 64 and 512 embedding dimensions across all datasets.

%we demonstrate the superiority of our proposed method by comparing the performance in  on image retrieval tasks.

\subsection{Qualitative Results}
We further demonstrate the superiority of our method through qualitative results of image retrieval. 
Fig.~\ref{fig:fig3} presents image retrieval examples of Proxy-Anchor loss incorporating L2A-NC and those of the vanilla Proxy-Anchor.
It can be shown in the examples that results of the vanilla Proxy-Anchor are often incorrect and focusing more on backgrounds rather than target objects, and L2A-NC enables retrieve correct images regardless of backgrounds.
% Interestingly, the vanilla version failed even though it successfully retrieved images whose background is more similar to query images than those from our combined model. 
Also, the vanilla version sometimes failed to retrieve even a single correct image for both of the Cars-196 and SOP datasets. 
Even in these cases, the version incorporating L2A-NC retrieved correct images although colors or viewpoints of target objects in these images are substantially different from that of the query. 
We would argue that L2A-NC functions as desired to regularize the vanilla method not to be biased towards certain prevailing features in the original dataset (\eg, background, the color of an object, and viewpoint) by augmenting novel classes unavailable in the original data. %\suhac{not very clear}


% We further demonstrate the superiority of our method on qualitative results for the image retrieval task. As shown in Fig.~\ref{fig:fig3}, the combination of our L2A-NC and Proxy-Anchor~\cite{kim2020proxy} is compared with the vanilla Proxy-Anchor.
% First, in the first row, most of the results of vanilla Proxy-Anchor are incorrect while our combined one retrieved all correct images. Interestingly, vanilla method failed even though it successfully retrieved images whose background is more similar to query images than those from our combined model. Even worse, vanilla one failed to retrieve even one correct result for both Cars-196 and SOP datasets. Whereas, our combined one retrieved correct images whose color or viewpoint is different from that of query images. We argue that our L2A-NC functions well to regularize the vanilla method not to be biased certain prevailing features in the original dataset (\eg, background, the color of an object, and viewpoint) by augmenting novel classes unavailable in the original data.

\begin{table}[]
    \tiny
    \centering
    
    \begin{tabular}{ccc}
    
    \begin{minipage}{.3\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc}
        \hline
        
        Dataset & +0\% & +25\% & +50\% & +100\% & +200\% \\
        \hline
        
        CUB & 69.1 & 69.3 & 69.6 & 69.5 & \textbf{69.7} \\
        SOP & 79.2 & 79.3 & 79.5 & 79.5 & \textbf{79.9} \\
        In-Shop & 91.9 & 92.0 & 92.2 & 92.2 & \textbf{92.3} \\
        \hline
        \end{tabular}
        }
    \end{minipage} &
    
    \begin{minipage}{.3\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccc}
        \hline
        Dataset  & Vanilla & L2A-EC & L2A-NC (Ours) \\
        \hline %\cline{2-5}
        CUB  & 69.1  & 69.2 & \textbf{69.7}      \\
        CARS & 86.4 & 86.8  & \textbf{87.9}   \\
        \hline
        \end{tabular}
        }
    \end{minipage} &
    
    \begin{minipage}{.3\linewidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c|c|c}
        \hline
        $\lambda_{div} $ & Norm-softmax & Arcface & Proxy-Anchor \\
        \hline %\cline{2-5}
        
        0.1 & 85.9 & 85.7 & 87.6  \\
        1.0 & \textbf{86.0} & \textbf{86.0} & \textbf{87.9}  \\
        10.0 & 85.7 & 85.5 & 87.5  \\
        \hline
        \end{tabular}
        }
    \end{minipage} &

    (a) Recall@1 versus the number of novel
classes. & (b) Comparison between L2A-EC and L2A-NC in Recall@1. & (c) Effect of $\lambda_{div} $ to retrieval performance in Recall@1.

    \end{tabular}
    %}
    \caption{Ablation studies on proposed L2A-NC. (\textbf{a}) includes something; (\textbf{b}) includes something; (\textbf{c}) includes something }
    \label{tab:my_label}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{new_figure/figure1_3_2.pdf}
%   \includegraphics[width=\columnwidth]{figure/fig4_5.pdf}
  \vspace{-2mm}
   \caption{
   $t$-SNE visualization of the learned embedding space. 
   (a) Embedding vectors of both real and novel classes. (b) Embedding vectors of novel classes only.
%   (a) Comparison of real and novel embedding vectors. (b) Comparison between novel embedding vectors
   }
    \label{fig:fig4}
\end{figure*}

\subsection{In-depth Analysis on L2A-NC}

\vspace{1mm}
\noindent \textbf{Impact of the number of novel classes.}
Thanks to the architecture of our conditional generator, L2A-NC can define and synthesize an arbitrary number of novel classes. 
% Intuitively speaking, we can conjecture that more novel classes seem to bring more performance boost. 
To investigate the impact of the number of novel classes, we evaluate the performance of L2A-NC incorporated with proxy-based losses while varying the number of novel classes. 
As shown in Fig.~\ref{fig:fig5}, the performance increases by adding more novel classes to some degree, but there is an upper bound of the effectiveness; 
it is natural since too many novel classes may prevent the embedding model from understanding relations between classes, leading to unstable training.
In experiments, we fixed the number of novel classes per dataset: 200\% of the number of existing classes for the CUB-200-2011 and Cars-196 datasets, and 25$\%$ for the SOP dataset.


\vspace{1mm}
\noindent \textbf{Importance of generating novel classes.}
To demonstrate that our performance boost is attributed to the augmentation of novel classes and their embedding vectors, we compare L2A-NC with its variant that produces synthetic embedding vectors of \textit{existing classes}; we call it L2A-EC (Learning to Augment Existing Classes).
% To prove that our performance boost is attributed to the augmented novel classes and their embedding vectors, we compare L2A-NC with the generator-based baseline that produces synthetic embedding vectors of \textit{existing classes} via optimizing the specific proxy-based loss, and we call it L2A-RC (Learning to Augment Real Classes).
%
L2A-NC and L2A-EC are incorporated with Proxy-NCA and Proxy-Anchor losses, and compared on the CUB-200-2011 dataset in terms of retrieval performance. 
As shown in Table~\ref{tab:tab2}, L2A-EC made marginal or no improvement while L2A-NC enhanced performance for both of the proxy-based losses. 
These results are consistent with our hypothesis that embedding vectors of novel classes unavailable in the original dataset would provide richer supervisory signals than those of existing classes.
% We would argue that these results demonstrate the effectiveness of \emph{augmenting novel classes} unavailable in the original dataset.

% On the CUB-200-2011 dataset, Recall@$1$ is evaluated for comparison and Proxy-NCA~\cite{movshovitz2017no} and Proxy-Anchor~\cite{kim2020proxy} are chosen as baseline loss functions. As shown in Tab.~\ref{tab:tab2}, L2A-RC either shows somewhat marginal performance improvement compared to L2A-NC or does little to help vanilla methods. This is consistent with our hypothesis that embedding vectors of novel classes unavailable in the original dataset would provide richer signals than those of existing classes.

%\usepackage{caption}
\begin{table}
\tiny
%\centering
\begin{minipage}[c]{0.5\textwidth}
\centering
\begin{tabular}{l|c}
\hline
Class pair  & Mean of minimum KL divergence \\
\hline
Train--Test   & 56.7     \\
Novel--Test   & \textbf{27.9}     \\
\hline
\end{tabular}
\caption{Ablation studies on proposed L2A-NC.}
\end{minipage}
\begin{minipage}[c]{0.5\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c}
\hline
Method  & sec / iter \downarrow &  \# of parameters \downarrow \\
\hline %\cline{2-5}
Vanilla  & 0.28  & 11.85M \\
PS~\cite{gu2020proxy} & 0.37 & 11.85M  \\
Ours & 0.43 & 12.24M  \\
\hline
\end{tabular}
}
\caption{Ablation studies on proposed L2A-NC.}
\end{minipage}
\end{table}

\iffalse
\begin{table}
\centering
\begin{tabular}{l|c}
\hline
Class pair  & Mean of minimum KL divergence \\
\hline
Train--Test   & 56.7     \\
Novel--Test   & \textbf{27.9}     \\
\hline
\end{tabular}
\caption{Quantitative analysis on how closely training and novel classes approximate unseen test classes.
% in the mean of minimum KL divergence between classes.
}
\label{tab:tab3}
\end{table}
\fi


\vspace{1mm}
\noindent \textbf{Hyperparameter ablation study.}

\vspace{1mm}
\noindent \textbf{\textit{t}-SNE visualization.}

\vspace{1mm}
\noindent \textbf{Training complexity.}


\vspace{1mm}
\noindent \textbf{Relation between novel classes and test classes.}
Recall that metric learning aims to find an embedding space well generalizable to unseen classes.
% The final goal of metric learning is to generalize the learned embedding space to unseen classes. 
% A way to demonstrate that the novel classes we generate affect the generalization is to investigate the relation between novel and unseen test classes.
% A way to demonstrate that the novel classes we generate affect the generalization is to investigate the relation between novel and unseen test classes.
% The way to demonstrate that the novel classes we generate affect the generalization on the unseen classes is to investigate the relation between two classes.
To demonstrate that the novel classes we generate affect the generalization, we investigate how well the novel and unseen test classes are aligned to each other in the learned embedding space.
Specifically, we quantify the degree of alignment through KL divergence: Each novel class is first matched with its nearest test class with the minimum KL divergence, then the minimum divergence values of all novel classes are averaged. 
% For this purpose, we quantify the relation through KL divergence.
% Specifically, each novel class is first matched with its nearest test class with the minimum KL divergence, then the minimum divergence values are averaged over all novel classes. 
We measure this score for training classes as well for comparison.
The results in Table~\ref{tab:tab3} demonstrate that novel classes better approximate test classes than training classes even though the conditional generator of L2A-NC is not aware of test data; this suggests that the proposed method has a potential to improve the generalization of the learned embedding space. 

% Although our novel classes are synthesized being unaware of the existence of test classes, it would be interesting to investigate the relations between novel classes and test classes. For example, if two classes are near each other, though it is just a coincidence, the existence of novel classes may become a sort of hints for the embedding network to learn features that are well-generalized for test classes.

% To this end, we measure KL divergence between these two classes, which is presented in Tab.~\ref{tab:tab3}. 

% a pair of novel class between two classes to get a sense of their relations, which is presented in Tab.~\ref{tab:tab3}.

% To this end, we quantify KL divergence between two classes to get a sense of their relations, which is presented in Tab.~\ref{tab:tab3}.

% Even though it is a coincidence, novel classes may give hint to if two classes are near each other.

% If two classes are near each other, though it is a just a coincidence, novel classes may give the embedding network a hint to be  

% that has an extremely large number of classes. 


% Thanks to the architecture of our conditional generator, L2A-NC can define and synthesize an arbitrary number of novel classes. Intuitively speaking, we can conjecture that more novel classes seem to bring more performance boost. To investigate the impact of the number of novel classes, we conduct an ablation study on Recall@1 with varying number of novel classes. As shown in Fig.~\ref{fig:fig4}, the performance increases to some degree along with the ratio of novel classes. This is in line with our motivation. However, there also seems to be a limit to maximize the performance. It is also natural because too many classes may prevent the embedding function from understanding relations between classes, leading to unstable training. Note that we have fixed this ratio of novel classes for each dataset; 200$\%$ for CUB-200-2011 and Cars-196, and 25$\%$ for SOP.

==> stage1_version/backup_table/backup2_4_table1.tex <==
\begin{table*}[!t]
    \centering
    \begin{tabular}{ll | c c c | c c c } %| c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{2}{l|}{\multirow{}{Recall@$K$}} &
    \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c}{Cars-196}
    \\ \cline{3-8}
    
    %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100 
    \multicolumn{2}{l|}{} & 1 & 2 & 4 & 1 & 2 & 4 % & 1 & 10 & 100 
    \\ \hline
    
    %Margin$^{128}$~\cite{sampling_matters} & 63.6 & 74.4 & 83.1 & 79.6 & 86.5 & 91.9 & 72.7 & 86.2 & 93.8 &
    \multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}& 57.1 & 68.8 & 78.7 & 81.4 & 88.0 & 92.7 &
    \multicolumn{1}{l|}{RLL-H~\cite{wang2019ranked}} & \multicolumn{1}{l|}{BN$^{512}$} & 57.4 & 69.7 & 79.2 & 74.0 & 83.6 & 90.1 &
    \multicolumn{1}{l|}{MS~\cite{wang2019multi}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.7 & 77.0 & 86.3 & 84.1 & 90.4 & 94.0 & 
    \hline
    %\multicolumn{1}{l|}{ProxyGML~\cite{Zhu2020ProxyGML}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 77.6 & 86.4 & 85.5 & 91.8 & 95.3 & 78.0 & 90.6 & 96.2 &
    \multicolumn{1}{l|}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.1 & 76.1 & 85.0 & 83.7 & 90.4 & 94.1 &
    \multicolumn{1}{l|}{Proxy-NCA + PS~\cite{gu2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.4 & 76.8 & 85.1 & 84.5 & 90.8 & 94.4 &
    \multicolumn{1}{l|}{Proxy-NCA + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{67.7} & \textbf{77.9} & \textbf{86.1} & \textbf{85.6} & \textbf{91.6} & \textbf{95.3} & 
    \hline
    \multicolumn{1}{l|}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.4 & 76.4 & 84.5 & 84.5 & 90.7 & \textbf{94.5} &
    \multicolumn{1}{l|}{SoftTriple + PS~\cite{gu2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.5 & 75.3 & 83.2 & 84.7 & 90.3 & 94.0 &
    \multicolumn{1}{l|}{SoftTriple + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{66.7} & \textbf{77.1} & \textbf{85.1} & \textbf{85.5} & \textbf{91.0} & 94.4 & 
    \hline
    \multicolumn{1}{l|}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.3 & 76.8 & 84.7 & 84.9 & 90.5 & 94.3 &
    \multicolumn{1}{l|}{SoftTriple + PS~\cite{gu2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 76.8 & 85.1 & 85.3 & 91.0 & \textbf{94.8} &
    \multicolumn{1}{l|}{SoftTriple + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{67.9} & \textbf{78.2} & \textbf{85.7} & \textbf{85.9} & \textbf{91.1} & 94.7 & 
    \hline
    \multicolumn{1}{l|}{Proxy-Anchor~\cite{kim2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 68.4 & 79.2 & 86.8 & 86.1 & 91.7 & 95.0 & 
    \multicolumn{1}{l|}{Proxy-Anchor + PS~\cite{gu2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 69.2 & 79.5 & \textbf{87.2} & 86.9 & \textbf{92.4} & 95.2 & 
    \multicolumn{1}{l|}{Proxy-Anchor + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{69.6} & \textbf{79.8} & 86.9 & \textbf{87.7} & 92.3 & \textbf{95.5} & 
    \hline
    \end{tabular}
    \vspace{0.1mm}
    \caption{
        Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the CUB-200-2011, Cars-196 and SOP datasets. Superscripts denote embedding dimension. Backbones of embedding networks are fixed as Inception with Batch Norm abbreviated as BN.
        %"-" means the result is not available.
        }
    %\vspace*{-4mm}
    \label{tab:quant_all}
\end{table*}

==> stage1_version/backup_table/backup3_4_table1.tex <==
\begin{table*}[!t]
    \centering
    \begin{tabular}{llc | c c c | c c c } %| c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{3}{l|}{} &
    \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c}{Cars-196}
    \\ \cline{4-9}
    
    %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100
    %\multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}
    \multicolumn{1}{l}{Method} & \multicolumn{1}{c}{Batch} & \multicolumn{1}{c|}{Arch} & R@1 & R@2 & R@4 & R@1 & R@2 & R@4 % & 1 & 10 & 100 
    \\ 
    
    \iffalse
    \hline
    %Margin$^{128}$~\cite{sampling_matters} & 63.6 & 74.4 & 83.1 & 79.6 & 86.5 & 91.9 & 72.7 & 86.2 & 93.8 &
    \multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{480}& \multicolumn{1}{l|}{BN$^{512}$}& 57.1 & 68.8 & 78.7 & 81.4 & 88.0 & 92.7 &
    \multicolumn{1}{l|}{RLL-H~\cite{wang2019ranked}} & \multicolumn{1}{l|}{BS}& \multicolumn{1}{l|}{BN$^{512}$} & 57.4 & 69.7 & 79.2 & 74.0 & 83.6 & 90.1 &
    \multicolumn{1}{l|}{MS~\cite{wang2019multi}} & \multicolumn{1}{l|}{BS} &\multicolumn{1}{l|}{BN$^{512}$} & 65.7 & 77.0 & 86.3 & 84.1 & 90.4 & 94.0 & 
    \fi
    
    \hline
    %\multicolumn{1}{l|}{ProxyGML~\cite{Zhu2020ProxyGML}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 77.6 & 86.4 & 85.5 & 91.8 & 95.3 & 78.0 & 90.6 & 96.2 &
    \multicolumn{1}{l}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{c}{128} & \multicolumn{1}{l|}{BN$^{512}$} & 65.1 & 76.1 & 85.0 & 83.7 & 90.4 & 94.1 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c}{128} & \multicolumn{1}{l|}{BN$^{512}$} & 66.4 & 76.8 & 85.1 & 84.5 & 90.8 & 94.4 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c}{128} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{67.7} & \textbf{77.9} & \textbf{86.1} & \textbf{85.8} & \textbf{91.8} & \textbf{95.2} & 
    \hline
    
    \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{c}{32} & \multicolumn{1}{l|}{BN$^{512}$} & 65.4 & 76.4 & 84.5 & 84.5 & 90.7 & 94.5 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c}{32} & \multicolumn{1}{l|}{BN$^{512}$} & 65.5 & 75.3 & 83.2 & 84.7 & 90.3 & 94.0 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c}{32} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{66.7} & \textbf{77.1} & \textbf{85.1} & \textbf{85.5} & \textbf{91.2} & \textbf{94.6} & 
    \hline
    \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{c}{128} & \multicolumn{1}{l|}{BN$^{512}$} & 66.3 & 76.8 & 84.7 & 84.9 & 90.5 & 94.3 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c}{128} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 76.8 & 85.1 & 85.3 & 91.0 & 94.8 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c}{128} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{67.9} & \textbf{78.2} & \textbf{85.7} & \textbf{86.0} & \textbf{91.3} & \textbf{94.9} & 
    \hline
    \multicolumn{1}{l}{Proxy-Anchor~\cite{kim2020proxy}} & \multicolumn{1}{c}{180} & \multicolumn{1}{l|}{BN$^{512}$} & 69.1 & 78.9 & 86.1 & 86.4 & 91.9 & 95.0 & 
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c}{180} & \multicolumn{1}{l|}{BN$^{512}$} & 69.2 & 79.5 & \textbf{87.2} & 86.9 & 92.4 & 95.2 & 
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c}{180} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{70.0} & \textbf{79.7} & 86.8 & \textbf{87.7} & \textbf{92.5} & \textbf{95.3} & 
    \hline
    \end{tabular}
    \vspace{0.1mm}
    \caption{
        Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the CUB-200-2011, Cars-196 and SOP datasets. Superscripts denote embedding dimension. Backbones of embedding networks are fixed as Inception with Batch Norm abbreviated as BN.
        %"-" means the result is not available.
        }
    %\vspace*{-4mm}
    \label{tab:quant_all}
\end{table*}

==> stage1_version/backup_table/backup4_4_table1.tex <==
\iffalse
resizebox{\textwidth}{!}{%
  \begin{tabular}{cc}
    Knuth & Lamport
  \end{tabular}}
\fi

\begin{table*}[!t]
    \scriptsize
    %\tiny
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ll | c c c | c c c | c c c | c c c} %| c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{2}{l|}{} &
    \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c}{Cars-196} & \multicolumn{3}{|c}{SOP} & \multicolumn{3}{|c}{In-Shop}
    \\ \cline{3-14}
    
    %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100
    %\multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}
    \multicolumn{1}{l}{Method} & \multicolumn{1}{c|}{Batch} & R@1 & R@2 & R@4 & R@1 & R@2 & R@4 & R@1 & R@10 & R@100 & R@1 & R@10 & R@20 
    \\ 
    
    \hline
    
    
    %\multicolumn{1}{l|}{ProxyGML~\cite{Zhu2020ProxyGML}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 77.6 & 86.4 & 85.5 & 91.8 & 95.3 & 78.0 & 90.6 & 96.2 &
    \multicolumn{1}{l}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{c|}{128} & 65.1 & 76.1 & 85.0 & 83.7 & 90.4 & 94.1 & 78.1 & 90.0 & 95.9 & 90.0 & 97.7 & 98.4 &
    
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.4 & 76.8 & 85.1 & 84.5 & 90.8 & 94.4 & 79.1 & 90.6 & 95.9 & 91.4 & 98.0 & 98.7 &
    
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{67.7} & \textbf{77.9} & \textbf{86.1} & \textbf{85.8} & \textbf{91.8} & \textbf{95.2} & - & - & - & - & - & - &
    \hline
    
    
    \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{c|}{32} & 65.4 & 76.4 & 84.5 & 84.5 & 90.7 & 94.5 & 78.3 & 90.4 & 96.0 & - & - & - &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{32} & 65.5 & 75.3 & 83.2 & 84.7 & 90.3 & 94.0 & - & - & - & - & - & - &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{32} & \textbf{66.7} & \textbf{77.1} & \textbf{85.1} & \textbf{85.5} & \textbf{91.2} & \textbf{94.6} & - & - & - & - & - & - &
    \hline
    
    \multicolumn{1}{l}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{c|}{128} & 66.3 & 76.8 & 84.7 & 84.9 & 90.5 & 94.3 & 79.0 & 90.7 & 96.1 & 91.1 & 97.8 & 98.4 &
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{128} & 66.6 & 76.8 & 85.1 & 85.3 & 91.0 & 94.8 & 79.5 & 90.6 & 96.0 & 91.8 & 98.1 & 98.7 &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{128} & \textbf{67.9} & \textbf{78.2} & \textbf{85.7} & \textbf{86.0} & \textbf{91.3} & \textbf{94.9} & - & - & - &  - & - & - &  
    \hline
    \multicolumn{1}{l}{Proxy-Anchor~\cite{kim2020proxy}} & \multicolumn{1}{c|}{180} & 69.1 & 78.9 & 86.1 & 86.4 & 91.9 & 95.0 & 79.1 & 90.8 & 96.2 & 91.5 & 98.1 & \textbf{98.8} & 
    \multicolumn{1}{l}{+ PS~\cite{gu2020proxy}} & \multicolumn{1}{c|}{180} & 69.2 & 79.5 & \textbf{87.2} & 86.9 & 92.4 & 95.2 & 79.8 & 90.9 & \textbf{96.4} &  91.9 & 98.2 & \textbf{98.8} &
    \multicolumn{1}{l}{+ L2A-NC} & \multicolumn{1}{c|}{180} & \textbf{70.0} & \textbf{79.7} & 86.8 & \textbf{87.7} & \textbf{92.5} & \textbf{95.3} & \textbf{79.9} & \textbf{91.2} & 96.1 & \textbf{92.3} & \textbf{98.3} & 98.7 &
    %\fi
    
    \hline
    \end{tabular}
    }
    \vspace{0.1mm}
    \caption{
        Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the CUB-200-2011, Cars-196 and SOP datasets. Superscripts denote embedding dimension. Backbones of embedding networks are fixed as Inception with Batch Norm abbreviated as BN.
        %"-" means the result is not available.
        }
    %\vspace*{-4mm}
    \label{tab:quant_all}
\end{table*}

\iffalse
Best Epoch: 2
Best Recall@1: 79.9709
Best Recall@10: 91.2367
Best Recall@100: 96.1770
Best Recall@1000: 98.5885


Best Epoch: 68
Best Recall@1: 79.0073
Best Recall@10: 90.7904
Best Recall@100: 96.1373
Best Recall@1000: 98.6381

\fi

==> stage1_version/backup_table/backup_3_method.tex <==
% !TEX root = ./bmvc21.tex

\section{Our Approach}
\label{sec:method}

As a way to improve generalization of deep metric learning, we propose a new data augmentation method called L2A-NC, which augments the data by hallucinating embedding vectors of novel classes.
Our method learns and utilizes a conditional generative network that models novel classes and produces discriminative and realistic embedding vectors of them.
The synthetic embedding vectors could behave like those of unseen real classes, and be incorporated with any proxy-based metric learning losses to help them construct a more discriminative and better generalizable embedding space.
The overall framework of L2A-NC is illustrated in Fig.~\ref{fig:fig2}.

In the rest of this section, we briefly review the proxy-based metric learning losses, present details of the conditional generative model, and describe the training procedure incorporating L2A-NC with proxy-based losses.

\iffalse % suha--20210120
% Our goal in this paper is to learn an embedding space which is well-generalized to unseen classes. As a straightforward way to achieve this, we propose to augment novel classes and synthesize their embedding vectors unavailable in the original dataset. To this end, we learn a generative network that produces discriminative and realistic samples. Thanks to these features that encourage novel class data to behave like those of real class, our method can construct a more discriminative embedding space.

% The rest of this section briefly reviews the proxy-based metric learning, presents details of the conditional generator, and describes our training procedure which is applicable to various proxy-based metric learning models. Our overall framework is illustrated in Fig 2.
\fi

\subsection{Background: Proxy-based Losses}
%The objective of this paper is to build an embedding space robust on unseen classes. Formally, we learn an embedding network parameterized by 

Proxy-based losses are a relatively new category of metric learning loss functions. 
They are devised for training with low complexity by introducing the concept of proxies~\cite{movshovitz2017no}. 
Proxies are representatives of training classes and learned together with network parameters. 
The basic idea of proxy-based losses is to learn an embedding model by utilizing relations between samples and proxies, which represent global class information.

%\kmoonc{The proxy-based loss is optimized by associating embedding vectors with proxies which are introduced in proxy-based metric learning and learned as a part of network parameters. For example, Proxy-NCA~\cite{movshovitz2017no}, an initial proxy-based loss, associates an embedding vector which is an anchor with proxies to be closer to the positive proxy and far from the negative proxies. Recently proposed Proxy-Anchor~\cite{kim2020proxy} associates a proxy which is an anchor with embedding vectors}

%The aforementioned issue gives rise to the proxy-based losses, a relatively new category of loss functions, with \textit{proxies}~\cite{movshovitz2017no}. As representatives of training classes, proxies are optimized as a part of the network parameters. Since the number of proxies is commonly much more addressable than that of training tuples, these losses can reduce both training complexity and convergence time by associating a proxy as a positive/negative sample~\cite{movshovitz2017no} or an anchor~\cite{kim2020proxy}.

Suppose that we aim to learn an embedding network $f$ parameterized by $\theta_{f}$ and proxies $P=[ p_{1}, p_{2}, \cdots{}, p_{C} ]$.
Let $X = [ x _{1}, x_{2}, \cdots{}, x_{N} ]$ be embedding vectors (\ie, the outputs of $f$) and $ Y = [ y_{1}, y_{2}, \cdots{}, y_{N}]$ be their corresponding labels, where $ y_{i} \in{ \{ 1, 2, .., C \} } $. 
A proxy-based loss optimized with respect to $\theta_{f}$ and $P$ are denoted by $J_{met}( X, Y, P)$.

% Formally, we learn an embedding network $f$ parameterized by $\theta_{f}$ and proxies $P=[ p_{1}, p_{2}, \cdots{}, p_{C} ] $. We also denote embedding vectors as $ X = [ x _{1}, x_{2}, \cdots{}, x_{N} ] $ and corresponding labels $ Y = [ y_{1}, y_{2}, \cdots{}, y_{N}]$, where $ y_{i} \in{ \{ 1, 2, .., C \} } $. Then, the specific proxy-based loss $J_{met}$ optimized with the embedding network and proxies is formulated as:
% \begin{equation}
% J_{met}( X, Y, P).
% \label{eqn:j_met}
% \end{equation}

Despite their improved performance in accuracy and speed, proxy-based losses can be further enhanced in the sense that they are inherently limited only to training classes, which would hamper generalization of the learned embedding space to unseen class data. 
From this perspective, this paper proposes a new data augmentation method to synthesize novel classes and their embedding vectors. 

% Despite its recent advances, however, the limited number of classes available in training may hamper the generalization of the embedding model since we cannot access unseen classes. From this perspective, we argue that there exists further room for performance boosting via data augmentation. Therefore, in this paper, we propose a new data augmentation approach to synthesize novel classes and their embedding vectors.

%To enlarge inter-class variation and compress intra-class variation, this proxy-based loss associates embedding vectors and proxies, and is optimized cooperatively by the embedding network and proxies. However, since we cannot access unseen classes data, the limited number of classes available in training may hamper generalization of the embedding model.

% \suhac{why existing augmentation techniques cannot be incorporated with proxy-based losses}


\iffalse
\subsection{Problem Formulation}
Formally, we denote a mini-batch of data points as $ D = [ d _{1}, d_{2}, \cdots{}, d_{N} ] $ and corresponding labels $ Y = [ y_{1}, y_{2}, \cdots{}, y_{N}]$, where $ y_{i} \in{ \{ 1, 2, .., C \} } $. The objective of deep metric learning is to learn an embedding function $ f : \boldsymbol{\mathcal{D}} \rightarrow{} \boldsymbol{\mathcal{X}} $ from the data space to the embedding space well so that it can reflect the semantic distances between input tuples. Namely, embedding vectors are from $ f $ as:
\begin{equation}
X = f( D )
\end{equation}

Different from pair-based losses, proxy-based losses introduce \textit{proxies}~\cite{movshovitz2017no,kim2020proxy} as representatives of each class, which are denoted as $P=[ p_{1}, p_{2}, \cdots{}, p_{C} ] $. Then, the parameters of the embedding function and the proxies are updated based on a given proxy-based loss $J_{m}$:

%In most frameworks of deep metric learning, parameters of the embedding function $ \theta_{f} $ are updated based on a given loss function $ J_{m} $:

%\DeclareMathOperator*{\argminA}{arg\,min} % Jan Hlavacek
%\DeclareMathOperator*{\argminB}{argmin}   % Jan Hlavacek
%\DeclareMathOperator*{\argminC}{\arg\min}   % rbp
%\newcommand{\argminD}{\arg\!\min} % AlfC

\newcommand{\argminD}{\arg\min} % AlfC

\begin{equation}
\min_{\theta_{f}}J_{m}(X, Y, P).
\end{equation}

In this paper, motivated by the main objective of deep metric learning to construct an embedding space that is robust on unseen classes, we aim to shed new light on achieving this goal via augmenting training classes and corresponding embedding vectors to exploit more diverse signals.%, which is orthogonal to existing approaches.

\fi

\subsection{Conditional Generator}

%Recent advances in deep metric learning have relied heavily on the loss functions or attempted to produce gradients of large magnitudes via hard sample mining. However, all of these approaches have a limitation that they are rather limited to a given training dataset. Inspired by the main objective of deep metric learning to learn an embedding space which is robust on unseen classes, we aim to shed light on 

%To define novel classes and generate their own embedding vectors, we introduce a conditional generator $ G $ which generates embedding vectors conditioned on sampled novel class labels $ \boldsymbol{\tilde{\mathrm{L}}} $ = [$ \tilde{l_{1}}, \tilde{l_{2}}, \cdots{}, \tilde{l_{n}}$], where $ \tilde{l_{i}} \in{ \{ C+1, C+2, .., C+\tilde{C} \} } $ and random variables $ \boldsymbol{z} \sim \mathcal{N}(0,\,\boldsymbol{\mathrm{I}}) $ that represent inter-class variation between novel classes and intra-class variation in each novel classes, respectively, as:

%Note that our generator does not produce real class data unlike existing generative models such as conditional generative adversarial networks although its architecture seems similar to theirs.
To synthesize novel classes, we learn their proxies $ \tilde{P}=[ p_{C+1}, p_{C+2}, \cdots{}, p_{C+\tilde{C} } ] $  and a conditional generator $ g $ which produces an embedding vectors of a novel class given its label $ \tilde{y} \in{ \{ C+1, C+2, .., C+\tilde{C} \} } $ and a random noise $z$ for stochastic generation:%random noise $z \sim \mathcal{N}(0,\, \mathbb{1})\ $ for stochastic generation as :
\begin{equation}
\tilde{x} = g(\tilde{y}, z).
\end{equation}
%where $ \tilde{Y} $ denotes our defined novel class labels, where $ \tilde{y}_{i} \in{ \{ C+1, C+2, .., C+\tilde{C} \} } $, $\tilde{X}$ denotes the corresponding embedding vectors, and $z$ denotes the latent variables. 
The generator consists of 4 fully connected layers, and is conditioned on the class label $\tilde{y}$ via conditional batch normalization layers~\cite{de2017modulating} which are placed between every pair of fully connected layers and transform intermediate features in a class-wise manner.
% supply parameters of batch normalization on external data which is the label information in our case.
%Specifically, the class label is injected via the conditional batch normalization layers~\cite{de2017modulating} which supply parameters of batch normalization~\cite{batchnorm} on the external data which is the class label in our case.

%the generator is fed with the randomly sampled latent variables which introduce stochastic generation, and is conditioned on the label via the conditional batch normalization layers~\cite{de2017modulating} which supply parameters of batch normalization~\cite{batchnorm} on the external data which is the class label in our case.

%Note that our generator augments classes that do not exist in the given dataset, which has the potential to enhance the training procedure compared to previous sample generation methods limited to the synthesis of known class samples.
Along with this conditional generation process, it is necessary to regularize our generator to produce realistic embedding vectors which are not far from the distribution of real embedding vectors; this is in line with previous work on data augmentation for deep metric learning~\cite{Schroff2015,Duan_2018_CVPR,Zheng_2019_CVPR}.
% this is in line with several studies~\cite{Schroff2015,Duan_2018_CVPR,Zheng_2019_CVPR}.
Furthermore, novel classes have to be discriminative so that they become diverse and independent to each other  like real classes of the original dataset.
% Furthermore, novel classes are encouraged to be synthesized discriminatively from each other not to act as a single class but to play the role of each independent class, which ends up providing diverse training classes to the embedding function.

To guarantee that our generator produces realistic and discriminative embedding vectors, we introduce two loss functions for its training: A divergence loss and a proxy-based loss. The divergence loss is embodied by a divergence measure $d$ between two sets of embedding vectors.
% detailed below. 
The generator is encouraged to fit its generated distributions in between those of real embedding vectors by minimizing the following divergence loss:
\begin{equation}
J_{div}( X, \tilde{X}) = d( X, \tilde{X}).
\label{eq:div_loss}
\end{equation}
Note that the loss is optimized with respect to $\tilde{X}$ only and does not back-propagate its gradients to $X$.
%where $ d(\cdot,\cdot) $ is a divergence measure which our generator aims to minimize.

As demonstrated in literature on generative models~\cite{genevay2018learning,martin2017wasserstein}, a good candidate for the divergence measure $d$ in Eq.~\eqref{eq:div_loss} is the Wasserstein distance, which allows $J_{div}$ to be statistically consistent~\cite{salimans2018improving}.
% \kmoonc{Inspired by recent progress of the Wasserstein distance in generative models~\cite{martin2017wasserstein,genevay2018learning} and its related work~\cite{zhou2020learning,liu2020semantic}, we design the divergence measure $d$ based on this distance to make $ J_{div}$  statistically consistent~\cite{salimans2018improving}.}
%
%
%and empirically found that it is more effective in reducing the discrepancy from the real embedding distribution than other techniques such as generative adversarial networks thanks to its statistically consistent and stable objective~\cite{salimans2018improving}.
The Wasserstein distance is defined by
\begin{equation}
    \mathcal{W}(p,q)= \inf_{\gamma \in \Pi_{(p,q)}} \mathbb{E}_{x_{p},\ x_{q} \sim \gamma } [c(x_{p},x_{q}) ],
\end{equation}
where $ \Pi{}(p,q) $ is the set of all joint distributions $ \gamma{}(x_{p},x_{q}) $ and $c(\cdot,\cdot)$ denotes a cost function. This distance is usually interpreted as the minimum cost to turn the distribution $ q $ into the distribution $ p $. However, since the optimization problem in Eq. (5) is generally intractable when using the Wasserstein directly, one can instead consider the entropy-regularized Wasserstein distance~\cite{cuturi2013sinkhorn}:
\begin{equation}
    \mathcal{W}_{\textrm{sinkhorn}}(p,q)= \inf_{\gamma \in \Pi_{\beta(p,q)}} \mathbb{E}_{x_{p},\ x_{q} \sim \gamma } [ c(x_{p},x_{q}) ],
\end{equation}
where $\Pi_{\beta}$ is restricted to distributions with entropy of at least some constant $\beta$. In addition, to evaluate the distance on given mini-batches of $X_{p}$, $X_{q}$, \textit{Sinkhorn AutoDiff}~\cite{genevay2018learning} is proposed as an approximate of the distance as
%In addition, \cite{genevay2018learning} proposes to approximate this distance to be evaluated on mini-batches of $X_{p}$, $X_{q}$, which is called \textit{Sinkhorn AutoDiff} and defined as:
\begin{equation}
    \mathcal{W}_{c}( X_{p}, X_{q})=\inf_{M \in \mathcal{M} } \Tr [M \odot  C  ],
\end{equation}
where the cost function $c$ becomes the cost matrix $C$, where $C_{i,j}=c(x^{p}_{i}, x^{q}_{j})$, and the coupling distribution $ \gamma $ becomes the soft matching matrix $M$ whose all rows and columns sum to one. Despite its strength of being able to perform efficient optimization on GPUs, its gradients become no longer an unbiased gradient estimator when using mini-batches. Therefore, to design $d$ of Eq.~\eqref{eq:div_loss}, we finally resort to \textit{Mini-batch Energy Distance}~\cite{salimans2018improving} which results in unbiased mini-batch gradients and is given by
\begin{equation}
\begin{aligned}
%\begin{split}
d(X, \tilde{X}) = & 2\mathbb{E}[\mathcal{W}_{c}(X_{1}, \tilde{X}_{1}) ] - \mathbb{E}[\mathcal{W}_{c}(X_{1}, X_{2})] \\ & -\mathbb{E}[\mathcal{W}_{c}(\tilde{X}_{1}, \tilde{X}_{2})],
\end{aligned}
%\end{split}
\end{equation}
where $X$ divided into $ X_{1} $ and $ X_{2} $ is a mini-batch from real data and $\tilde{X}$ divided into $\tilde{X}_{1} $ and $\tilde{X}_{2} $ is a mini-batch from generated data. For a cost function $c$, we adopt the cosine distance between two embedding vectors.
%\begin{equation}
 %   asdf%c( x, \tilde{x} )= 1 - ||x||| over ||x||. %\inf_{M \in \mathcal{M} } \Tr [\ M \odot  C  ]\ ,
%\end{equation}
%By minimizing $ J_{div} $ equipped with Eq. (7), our generator encourages the distribution of synthetic classes to be as close as possible to that of real ones.

In addition, we train the generator to produce discriminative embedding vectors. 
To this end, the generator aims to minimize a proxy-based loss that takes not only embedding vectors of novel classes but also those of real classes so that the augmented embedding vectors help increase inter-class variation while reducing intra-class variation of both real and synthetic classes.
Formally, the objective is given by 
% This joint training phase is the most important in our L2A-NC, the objective is formulated as:
% In addition, we train the generator to produce discriminative embedding vectors. To be specific, the generator aims to minimize the proxy-based loss which incorporates not only embedding vectors of novel classes but also those of real classes. This joint training phase is the most important in our L2A-NC, the objective is formulated as:
\begin{equation}
 J_{met}( X\cup\tilde{X}, Y\cup\tilde{Y}, P\cup\tilde{P}).
\end{equation}

%\textcolor{blue}{Inspired by recent progress of the Wasserstein distance as also known as optimal transport distance in generative models~\cite{martin2017wasserstein, genevay2018learning, salimans2018improving, shaham2019singan, wu2019sliced, deshpande2019max} and its related work~\cite{courty2016optimal, su2015optimal, zhou2020learning, liu2020semantic, xu2019gromov}, we adopt this distance as divergence measure and empirically found that it is more effective in reducing the discrepancy from the real embedding distribution than other techniques such as generative adversarial networks thanks to its statistically consistent and stable objective~\cite{salimans2018improving}. The wasserstein distance is defined by:
%\begin{equation}
%    W_{c}(p,q)= \inf_{\gamma \in \Pi_{(p,q)}} \mathbb{E}_{x_{p},\ x_{q} \sim \gamma } [\ c(x_{p},x_{q}) ]\ ,
%\end{equation}
%where $ \Pi{}(p,q) $ is the set of all joint distributions $ \gamma{}(x_{p},x_{q}) $ and $c(\cdot,\cdot)$ denotes a cost function. However, since the optimization problem in Eq. 5 is generally intractable, we resort to the entropy-regularized optimal transport distance, referred to the sinkhorn distance~\cite{cuturi2013sinkhorn}. In addition, \cite{genevay2018learning} proposes to approximate this distance to be evaluated on mini-batches of $\textbf{X}_{a}$, $\textbf{X}_{b}$, which is called \textit{Sinkhorn AutoDiff} and defines as:
%\begin{equation}
%    W_{c}( \boldsymbol{\mathrm{X}}_{a},\boldsymbol{\mathrm{X}}_{b})=\inf_{M \in \mathcal{M} } \Tr [\ M \odot  C  ]\,
%\end{equation}
%where the soft matching matrix $ M $ and the cost matrix $ C $ replace the coupling distribution $ \gamma $ and the cost function $ c $, respectively in Eq. 5. In spite of its advantage which is that the optimization over $ M $ can be tractable on the GPU with the Sinkhorn algorithm, it becomes no longer an unbiased gradient estimator~\cite{bellemare2017cramer}. Therefore, we finally design $ L_{div}$ as the \textit{Mini-batch Energy Distance}~\cite{salimans2018improving} which results in unbiased mini-batch gradients. \begin{equation}
%d( p, q) = 2\mathbb{E}[W_{c}(\boldsymbol{\mathrm{X}}_{a}, \boldsymbol{\mathrm{X}}_{b}) ] - \mathbb{E}[W_{c}(\boldsymbol{\mathrm{X}}_{a}, \boldsymbol{\mathrm{X}}_{a^{\prime}})] - \mathbb{E}[W_{c}(\boldsymbol{\mathrm{X}}_{b}, \boldsymbol{\mathrm{X}}_{b^{\prime}})],
%\end{equation}
%where $ \textbf{X}_{a} $ and $ \textbf{X}_{a^{\prime}} $ are independent mini-batches from the distribution $ p $ and $ \textbf{X}_{b} $ and $ \textbf{X}_{b^{\prime}} $ are independent %ones from the distribution $ q $. }

% Having obtained the augmented embeddings, we utilize a simultaneously trained generator to map them back to the feature space while preserving the label and augmented hardness.



%Having forced our generated sample distribution similar to the real sample distribution, now we focus on the inter-class separability between our novel classes. This is simply achieved by optimizing the metric learning loss since it is fundamentally designed to maximize inter-class variation and minimize intra-class variation. Therefore, we design $J_{novel}$ as the proxy-based loss with proxies of novel classes by
%\begin{equation}
%J_{novel} = J_{m}( \tilde{X}, \tilde{Y}, \tilde{P}),
%\end{equation}
%where $\tilde{X}$ denotes a mini-batch of novel-class embedding vectors, $\tilde{Y}$ denotes labels for each embedding vector, and $\tilde{P}=[p_{C+1}, p_{C+2}, \cdots{}, p_{C+\tilde{C}},]$ denotes proxies for novel classes.
%Note that Eq.~(8) achieves inter-class separability between our generated samples, not real samples.


%To define novel classes and generate their own embedding vectors, we introduce a conditional generator $ G $, which generates embedding vectors conditioned on sampled novel class labels $ l_{i}^{\prime} \in{ \{ C+1, C+2, .., C+C^{\prime} \} } $ and random variable $ z \sim \mathcal{N}(0,\,\mathcal{I}) $, which of each represent inter-class variation between novel classes and intra-class variation in novel classes, respectively. 

%maps sampled novel class labels to corresponding embedding vectors. as:


% G :  \mathcal{L}^{\prime} \times{} \mathcal{Z} \rightarrow{} \mathcal{Y} $, which generates embedding vectors conditioned on sampled novel class labels $ l_{i}^{\prime} \in{ \{ C+1, C+2, .., C+C^{\prime} \} } $ and random variables $ z_{i} \sim \mathcal{N}(0,\,\mathcal{I}) $, which of each represent inter-class variation between novel classes and intra-class variation in novel classes, respectively. Note that our generator does not produce real class data unlike existing generative models such as conditional generative adversarial networks although its architecture seems similar to theirs.

%Moreover, we aim for our generated samples to be informative signals to the target embedding network. To this end, we train our generator $ g $ to optimize 

%it is also worth noting that the augmented data should be generated in a way of giving sufficiently meaningful signals to the target embedding network. 

%It has been witnessed that the hard negatives whose distance is small from the anchor produce large gradients and alleviate the lack of informative samples for training. Similarly, we first train our generator to minimize the distribution divergence measure between the generated distribution and the real distribution (which will be detailed in Sec 3.2) so that our defined class distribution becomes hard for the real class distribution.


%Once we manipulate generated embeddings to be hard samples, next we aim to identify novel classes. Without the identification between these classes, they would act indistinguishably as a single class, although they consist of multiple classes, which ends up limiting the diversity of additional signals to be provided to the embedding network. Figure 2 shows our overall framework.

\iffalse
\begin{algorithm}[tb]
\caption{Learning to Augment Novel Classes (L2A-NC)}
\label{alg:algorithm}
\textbf{Input}: Real embedding vectors $ X $ whose labels are denoted as $Y$, novel-class labels $\tilde{Y}$, and random noise $Z$. \\
\textbf{Parameter}: Parameters of the embedding network $\theta_{f}$, parameters of the generator $\theta_{g}$, proxies for real classes $P$ and proxies for novel classes $\tilde{P}$ \\
% Parameters of 
\textbf{Output}: Parameters of the embedding network  $\theta_{f}$.

\begin{algorithmic}[1] %[1] enables line numbers
\STATE Pretrain $ \{ \theta_{f}, P \}$ using Eq.~\eqref{eq:eqn9}.
\STATE Initialize and pretrain $\{ \theta_{g}, \tilde{P} \}$ using Eq.~\eqref{eq:eqn10}.

% \FOR{$iter$=1 to $T$}
\WHILE{not reaching the max iterations}
    %\STATE Sample a mini-batch ($D, Y$).
    %\STATE Get real samples $X=f(D)$.
    %\STATE Sample novel-class labels $\tilde{Y}$, and latent variables $z$.
    \STATE Embed real embedding vectors $ X $ from the embedding network $f$.
    \STATE Generate embedding vectors of novel classes $\tilde{X}=g(\tilde{Y}, Z)$.
    \STATE Optimize $\{ \theta_{f}, \theta_{g}, P, \tilde{P} \}$ using Eq.~\eqref{eq:eqn11}.
    \STATE Optimize $\theta_{g}$ using Eq.~\eqref{eq:div_loss}.
% \ENDFOR
\ENDWHILE
\STATE \textbf{return} $\theta_{f}$
\end{algorithmic}
\end{algorithm}
\fi

% \input{_4_table2}



\subsection{Proxy-based Metric Learning with L2A-NC}
%, consisting of the embedding network, the proposed conditional generator, proxies for both real classes and novel classes, and several losses described above.
This section illustrates the overall pipeline of our method. 
We first pretrain the embedding function $f$ alone via a specific proxy-based loss $J_{met}$:
%
% In this section, we illustrate the overall framework of our method to augment novel classes and their embedding vectors so as to achieve our final goal which is to build an embedding space well-generalized to unseen classes. For the training procedure, we first pretrain the embedding function alone via a specific proxy-based loss $J_{met}$ as:
\begin{equation}
\min_{\theta_{f},P}J_{met}( X, Y, P).
\label{eq:eqn9}
\end{equation}
%
The conditional generator is also pretrained by the following optimization so as to prepare for generating realistic and discriminative embedding vectors:
% we also pretrain the generator to prepare for realistic and discriminative generation in advance as:
\begin{equation}
\min_{\theta_{g},\tilde{P}}J_{met}( \tilde{X}, \tilde{Y}, \tilde{P}) + \lambda_{div} J_{div}( X, \tilde{X}),
\label{eq:eqn10}
\end{equation}
where $\lambda_{div} $ is a hyperparameter to balance the two losses. 
In this pretraining stage for the generator, we exclude real embedding vectors when applying $J_{met}$ since synthetic embedding vectors that are not sufficiently trained yet could have a negative effect on those of real classes if they are trained together by $J_{met}$. 
% we find it pertinent to exclude real embedding vectors it would somewhat invalidate the final joint training phase if embedding vectors of novel classes become discriminative from those of real classes.

Finally, in the joint training phase, the two networks $f$ and $g$ are learned by optimizing the following common objective: 
\begin{equation}
\min_{\theta_{f},\theta_{g},P,\tilde{P}}J_{met}( X\cup\tilde{X}, Y\cup\tilde{Y}, P\cup\tilde{P}).
\label{eq:eqn11}
\end{equation}
In this phase also, we employ the divergence loss in Eq.~\eqref{eq:div_loss} to regularize the generator and ensure that it keeps producing realistic embedding vectors. 
% for the generator to ensure its realistic generation, though the embedding space changes at each iteration of the joint training phase. 

%Algorithm~\ref{alg:algorithm} summarizes the overall training procedure.

%For the training procedure, we first pretrain the embedding function alone via a specific proxy-based loss $J_{m}$. Next, we also pretrain proxies of novel classes and the generator to produce novel-class samples which are realistic and inter-class separable with the pretrained embedding network via $\tilde{J}_{gen}$:
%where $ \theta_{G} $, $ \theta_{n} $ and $\lambda_{div} $ are parameters of the generator, proxies for novel classes,
%where $\lambda_{div} $ is a hyperparameter to balance two losses. For $J_{novel}$, we find it pertinent to exclude real samples since generated samples that are already well-separated from real ones would not be quite useful in the joint training phase. Lastly, two networks are optimized together. In this joint training phase, the proxy-based loss for the embedding network is reformulated to include samples and proxies of novel classes as: 

%Thus, the embedding network and proxies for all classes are jointly trained with $J_{joint}$, which is our final goal to provide rich signals reflecting more diversified class relations. For the generator, we keep employing $ J_{div} $ to ensure realistic generation although the embedding space changes at each iteration. In addition, $J_{joint}$ is employed together. In other words, two networks conspire together to construct a well-clustered embedding space reflecting novel classes. Therefore, the objective of the generator in the joint training phase is as follows: 
%\begin{equation}
%J_{gen} = J_{joint} + \lambda_{div} J_{div}.
%\end{equation} Algorithm 1 describes the overall training %procedure.

%Our goal is to encourage the embedding network to exploit more diverse signals from our generated novel classes. However, while the embedding network is optimized with 

%\textbf{Generator} 

%\textbf{Embedding Network}


%\subsubsection{Generator Training}
%\subsubsection{Embedding Network Training}
%\subsection{Analysis}
%\subsubsection{OT Minimization}
%\subsubsection{DML for Generator}



==> stage1_version/backup_table/backup_4_table1_.tex <==
\begin{table*}[!t]
    \centering
    \begin{tabular}{ll|c c c |c c c |c c c}
    \hline
    %\multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196} & \multicolumn{3}{c}{SOP}\\ \cline{3-11} \multicolumn{2}{l|}{} &1 &2 &4 &1 &2 &4 &1 &10 &100 \\ \hline%
    %{}
    \multicolumn{2}{l|}{\multirow{2}{*}[-2mm]{Recall@$K$}} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{Cars-196}
       & \multicolumn{3}{c}{SOP}
    \\ \cline{3-11}
    
    %{Recall@\textit{K}} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100 
    \multicolumn{2}{l|}{} & 1 & 2 & 4 & 1 & 2 & 4 & 1 & 10 & 100 
    \\ \hline
    
    %Clustering~\cite{songCVPR17} & 48.2 & 61.4 & 71.8 & 58.1 & 70.6 & 80.3 & 67.0 & 83.7 & 93.2 &
    \multicolumn{1}{l|}{Clustering~\cite{songCVPR17}}& \multicolumn{1}{l|}{BN$^{64}$} & 48.2 & 61.4 & 71.8 & 58.1 & 70.6 & 80.3 & 67.0 & 83.7 & 93.2 &
    \multicolumn{1}{l|}{Smart Mining~\cite{Harwood_2017_ICCV}} & \multicolumn{1}{l|}{BN$^{64}$} & 49.8 & 62.3 & 74.1 & 64.7 & 76.2 & 84.2 & - & - & - & 
    \multicolumn{1}{l|}{Proxy-NCA~\cite{movshovitz2017no}} & \multicolumn{1}{l|}{BN$^{64}$} & 49.2 & 61.9 & 67.9 & 73.2 & 82.4 & 86.4 & 73.7 & - & - & 
    \multicolumn{1}{l|}{Proxy-NCA + L2A-NC} & \multicolumn{1}{l|}{BN$^{64}$} & 50.8 & 62.9 & 73.0 & 73.8 & 82.4 & 88.6 & 74.3 & 87.9 & 94.7 & 
    \multicolumn{1}{l|}{Proxy-Anchor~\cite{kim2020proxy} } & \multicolumn{1}{l|}{BN$^{64}$} & 61.7 & 73.0 & 81.8 & 78.8 & 87.0 & 92.2 & 76.5 & 89.0 & 95.1 & 
    \multicolumn{1}{l|}{Proxy-Anchor + L2A-NC} & \multicolumn{1}{l|}{BN$^{64}$} & \textbf{62.6} & \textbf{73.4} & \textbf{82.1} & \textbf{80.4} & \textbf{87.7} & \textbf{92.4} & \textbf{76.7} & \textbf{89.0} & \textbf{95.1} \\

    \hline
    %Margin$^{128}$~\cite{sampling_matters} & 63.6 & 74.4 & 83.1 & 79.6 & 86.5 & 91.9 & 72.7 & 86.2 & 93.8 &
    \multicolumn{1}{l|}{HTL~\cite{Ge2018DeepML}}& \multicolumn{1}{l|}{BN$^{512}$}& 57.1 & 68.8 & 78.7 & 81.4 & 88.0 & 92.7 & 74.8 & 88.3 & 94.8 &
    \multicolumn{1}{l|}{RLL-H~\cite{wang2019ranked}} & \multicolumn{1}{l|}{BN$^{512}$} & 57.4 & 69.7 & 79.2 & 74.0 & 83.6 & 90.1 & 76.1 & 89.1 & 95.4 &
    \multicolumn{1}{l|}{MS~\cite{wang2019multi}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.7 & 77.0 & 86.3 & 84.1 & 90.4 & 94.0 & 78.2 & 90.5 & 96.0 &
    %\multicolumn{1}{l|}{ProxyGML~\cite{Zhu2020ProxyGML}} & \multicolumn{1}{l|}{BN$^{512}$} & 66.6 & 77.6 & 86.4 & 85.5 & 91.8 & 95.3 & 78.0 & 90.6 & 96.2 &
    \multicolumn{1}{l|}{SoftTriple~\cite{Qian_2019_ICCV}} & \multicolumn{1}{l|}{BN$^{512}$} & 65.4 & 76.4 & 84.5 & 84.5 & 90.7 & 94.5 & 78.3 & 90.3 & 95.9 & 
    \multicolumn{1}{l|}{SoftTriple + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & 66.3 & 77.0 & 85.1 & 85.2 & 91.1 & 94.5 & 77.8 & 89.8 & 95.5 &
    \multicolumn{1}{l|}{Proxy-Anchor~\cite{kim2020proxy}} & \multicolumn{1}{l|}{BN$^{512}$} & 68.4 & \textbf{79.2} & \textbf{86.8} & 86.1 & 91.7 & 95.0 & 79.1 & 90.8 & 96.2 &
    \multicolumn{1}{l|}{Proxy-Anchor + L2A-NC} & \multicolumn{1}{l|}{BN$^{512}$} & \textbf{69.6} & 79.1 & 86.4 & \textbf{87.2} & \textbf{92.2} & \textbf{95.3} & \textbf{79.9} & \textbf{91.2} & \textbf{98.7} 
    \\ \hline
    \end{tabular}
    \vspace{0.1mm}
    \caption{
        Comparison with the state-of-the-art methods. Image retrieval performance is measured as Recall@K ($\%$) on the CUB-200-2011, Cars-196 and SOP datasets. Superscripts denote embedding dimension. Backbones of embedding networks are fixed as Inception with Batch Norm abbreviated as BN.
        %"-" means the result is not available.
        }
    \vspace*{-4mm}
    \label{tab:quant_all}
\end{table*}
